Greedy inference with structure-exploiting lazy maps

We propose a framework for solving high-dimensional Bayesian inference problems using \emph{structure-exploiting} low-dimensional transport maps or flows. These maps are confined to a low-dimensional subspace (hence, lazy), and the subspace is identified by minimizing an upper bound on the Kullback--Leibler divergence (hence, structured). Our framework provides a principled way of identifying and exploiting low-dimensional structure in an inference problem. It focuses the expressiveness of a transport map along the directions of most significant discrepancy from the posterior, and can be used to build deep compositions of lazy maps, where low-dimensional projections of the parameters are iteratively transformed to match the posterior. We prove weak convergence of the generated sequence of distributions to the posterior, and we demonstrate the benefits of the framework on challenging inference problems in machine learning and differential equations, using inverse autoregressive flows and polynomial maps as examples of the underlying density estimators.

==> arXiv v2/additional-details-blr.tex <==
\subsection{Additional details: Bayesian logistic regression}\label{app:example:blr}
Here we provide addition details and results for the Bayesian logistic regression problems discussed in \S \ref{sec:examples:blr}. We begin by further describing the UCI Parkinson's disease data set \cite{parkinsonsUCI}. The $500$ features we consider consist of the patient sex, and audio extensions from a patient recording. The data set includes data from $3$ independent recordings from $188$ Parkinson's disease patients and a control group of $64$ individuals, totaling $756$ observations in all. The low rank problem considers $20$ observations where we use observations from $20$ different individuals.

We imposed a non-informative prior of $\sfN(0,10^2 I_d)$ on the parameters. Samples from the prior can be transformed to match those of a standard normal distribution via a \emph{whitening} transformation, i.e.
\[
z \sim \sfN(0,10^2 I_d), \  Wz:= \frac{1}{10} z \sim \sfN(0,I_d),
\]
where we let $W$ denote this whitening operation. We consider the transformed posterior
\[
\widetilde{\pi}(x) \propto \sfL(W^{-1} x) \rho(x)
\]
where the prior has been replaced with a standard normal distribution. This whitened posterior relates to the true posterior by $\widetilde{\pi} = W_\sharp \pi$. We see that solving this transformed problem is equivalent to solving the original, and that working with this whitened problem directly exposes lazy structure by matching the form of \ref{eq:LazyMap_VS_Ridge}. A similar whitening process is followed for each of the numerical experiments.

Figure \ref{fig:app:blr:lr} shows mean performance metrics through out the training process for each of the maps considered. Each metric is computed with $500$ independent samples. For G3-IAF, the three lazy layers were trained for $5000$, $5000$ and $10000$ iterations, which can be seen as sharp decreases in the negative ELBO and trace diagnostics occur. In general we see faster convergence in terms of the number of iterations for maps using the lazy framework compared to the baselines.
\begin{figure}
	\centering
	\begin{subfigure}[b]{.49\textwidth}
		\includegraphics[width=\textwidth]{convergence-plots/blr_lr_elbos.pdf}
		\caption{Low rank - Negative ELBO}
		\label{fig:blr:lr:elbo}
	\end{subfigure}
	\hspace{2pt}
		\begin{subfigure}[b]{.49\textwidth}
		\includegraphics[width=\textwidth]{convergence-plots/blr_lr_elbos.pdf}
		\caption{Full rank - Negative ELBO}
		\label{fig:blr:fr:elbo}
	\end{subfigure}


	\begin{subfigure}[b]{.49\textwidth}
	\includegraphics[width=\textwidth]{convergence-plots/blr_lr_traces.pdf}
	\caption{Low rank - $\trace(H^{\text{B}})$}
	\label{fig:blr:lr:traces}
\end{subfigure}
	\hspace{2pt}
		\begin{subfigure}[b]{.49\textwidth}
		\includegraphics[width=\textwidth]{convergence-plots/blr_fr_traces.pdf}
		\caption{Full rank - $\trace(H^{\text{B}})$}
		\label{fig:blr:fr:traces}
	\end{subfigure}

	\begin{subfigure}[b]{.49\textwidth}
	\includegraphics[width=\textwidth]{convergence-plots/blr_lr_is_traces.pdf}
	\caption{Low rank - $\trace(H)$}
	\label{fig:blr:lr:is-traces}
\end{subfigure}
\hspace{2pt}
	\begin{subfigure}[b]{.49\textwidth}
	\includegraphics[width=\textwidth]{convergence-plots/blr_fr_is_traces.pdf}
	\caption{Full rank - $\trace(H)$}
	\label{fig:blr:fr:is-traces}
\end{subfigure}
%	\hspace{2pt}
%	\begin{subfigure}[b]{.29\textwidth}
%	\includegraphics[width=\textwidth]{convergence-plots/blr_lr_evs.pdf}
%	\caption{low rank eigenvalues}
%	\label{fig:blr:lr:eigvalues}
%\end{subfigure}
	\caption{
		Mean training plots for the low rank (left) and full rank (right) Bayesian logistic regression problems across $10$ optimization runs. $^*$The $x$-axes include the cost of forming the matrices $H_\ell$ to determine the subspace $U^{\ell}$ in terms of gradient evaluations. Each matrix is computed using $500$ gradient evaluations, the same cost as $5$ optimization steps.
	}
	\label{fig:app:blr:lr}
\end{figure}


%\begin{figure}
%	\centering
%	\begin{subfigure}[b]{.29\textwidth}
%		\includegraphics[width=\textwidth]{convergence-plots/blr_fr_elbos.pdf}
%		\caption{Negative ELBO}
%		\label{fig:blr:fr:elbo}
%	\end{subfigure}
%	\hspace{2pt}
%	\begin{subfigure}[b]{.29\textwidth}
%		\includegraphics[width=\textwidth]{convergence-plots/blr_fr_traces.pdf}
%	\caption{$\trace(H^{\text{B}})$}
%		\label{fig:blr:fr:traces}
%	\end{subfigure}
%	\hspace{2pt}
%	\begin{subfigure}[b]{.29\textwidth}
%		\includegraphics[width=\textwidth]{convergence-plots/blr_fr_is_traces.pdf}
%	\caption{$\trace(H)$}
%	\end{subfigure}
%%	\hspace{2pt}
%%	\begin{subfigure}[b]{.29\textwidth}
%%		\includegraphics[width=\textwidth]{convergence-plots/blr_fr_evs.pdf}
%%		\caption{full rank eigenvalues}
%%		\label{fig:blr:fr:eigvalues}
%%	\end{subfigure}
%	\caption{
%		Mean training plots for the full rank Bayesian logistic regression problem across $10$ optimization runs.
%	}
%	\label{fig:app:blr:fr}
%\end{figure}

==> arXiv v2/additional-details-bnn.tex <==
\subsection{Additional details: Bayesian neural network}\label{app:example:bnn}

In \S \ref{sec:examples:bnn} we considered a Bayesian neural network that is also used as a test problem in \cite{liu2016stein} and \cite{Detommaso2018}. Bayesian neural networks generate high dimension inference problems, where the parameter dimension is the number of parameters in the underlying neural network. We considered the UCI yacht hydrodynamics data set \cite{yachtrockUCI}. In our example, the parameter dimension is $581$, given an input dimension of $6$, one hidden layer of dimension $20$, and output layer of dimension $1$. We use sigmoid activation functions in the input and hidden layer, and a linear output layer. The prior on the model parameters is taken to be zero mean Gaussian with a variance of $100$.

Here we consider affine maps, i.e., maps of the form $T(x) = \mu + Lx$, where $L \in \R^{d \times d}$ denotes a lower triangular matrix and $\mu \in \R^d$ a constant vector. The approximate posteriors in this case are indeed Gaussian distributions with mean $\mu$ and covariance $\Sigma = L L^T$. We note that the final approximate posterior given by the G3-affine transport map is also Gaussian given that the composition of affine functions is affine. Therefore the performance benefits we see may come from avoiding sub-optimal minima of the KL divergence. We see stabler training in terms of the performance metrics in Figure \ref{fig:app:bnn}. For G3-affine, layers were trained for $5000$, $5000$ and $10000$ iterations, where we see sharp decreases in each of the diagnostics.
\begin{figure}
	\centering
	\begin{subfigure}[b]{.49\textwidth}
		\includegraphics[width=\textwidth]{convergence-plots/bnn_elbos.pdf}
		\caption{Negative ELBO}
		\label{fig:bnn:elbo}
	\end{subfigure}
	\hspace{2pt}
	\begin{subfigure}[b]{.49\textwidth}
		\includegraphics[width=\textwidth]{convergence-plots/bnn_traces.pdf}
	\caption{$\trace(H^{\text{B}})$}
		\label{fig:bnn:traces}
	\end{subfigure}
	\hspace{2pt}
	\begin{subfigure}[b]{.49\textwidth}
		\includegraphics[width=\textwidth]{convergence-plots/bnn_is_traces.pdf}
	\caption{$\trace(H)$}
		\label{fig:bnn:is-traces}
	\end{subfigure}
	\hspace{2pt}
	\begin{subfigure}[b]{.49\textwidth}
		\includegraphics[width=\textwidth]{convergence-plots/bnn_evs.pdf}
		\caption{Spectrum of $H^\text{B}_\ell$ before and after training each lazy layer.}
		\label{fig:bnn:eigvalues}
	\end{subfigure}
	\caption{
		(\subref{fig:bnn:elbo},\subref{fig:bnn:traces},\subref{fig:bnn:is-traces}) Mean training plots for the Bayesian neural network problem across $10$ optimization runs. $^*$The $x$-axes include the cost of forming the matrices $H_\ell$ to determine the subspace $U^{\ell}$ in terms of gradient evaluations. Each matrix is computed using $581$ gradient evaluations, approximately the same cost as $6$ optimization steps. (\subref{fig:bnn:eigvalues}) Analogous plot to Figure \ref{fig:blr_fullrank_eigenvalues} for the Bayesian neural network problem. The spectrum of the diagnostic matrices $H^{\text{B}}_\ell$ flatten and fall as the approximation to the posterior improves with each lazy layer.
	}
	\label{fig:app:bnn}
\end{figure}

==> arXiv v2/additional-details-ellipticPDE.tex <==
\subsection{Additional details: High-dimensional elliptic PDE inverse problem}\label{app:examples:elliptic}

\begin{figure}
  \centering
  \begin{subfigure}[b]{.29\textwidth}
    \includegraphics[width=\textwidth]{./elliptic-synthetic-solution.pdf}
    \caption{Solution $\Sc(\kappab^\star)$}
    \label{fig:ex:elliptic:true-solution}
  \end{subfigure}
  \hspace{2pt}
  \begin{subfigure}[b]{.31\textwidth}
    \includegraphics[width=\textwidth]{./elliptic-eig-mean.pdf}
    \caption{$\mathbb{E}[\kappab\vert\yb^\star]$}
    \label{fig:ex:elliptic:mean-log-kappa}
  \end{subfigure}
  \hspace{2pt}
  \begin{subfigure}[b]{.32\textwidth}
    \includegraphics[width=\textwidth]{./elliptic-eig-std.pdf}
    \caption{$\mathrm{Std}[\kappab\vert\yb^\star]$}
    \label{fig:ex:elliptic:std-log-kappa}
  \end{subfigure}
  \caption{
    Additional figures for the elliptic problem with
    unknown diffusion coefficient.
    Figure
    (\subref{fig:ex:elliptic:true-solution}) shows the solution $u$
    corresponding to the field in Figure \ref{fig:ex:elliptic:true-kappa}.
    Figures
    (\subref{fig:ex:elliptic:mean-log-kappa}) and
    (\subref{fig:ex:elliptic:std-log-kappa})
    show the mean and the standard deviation of the posterior distribution.
  }
  \label{fig:app:elliptic}
\end{figure}

Here we explain how the numerical discretization of the PDE enters
the Bayesian inference formulation.
We denote by $\Sc$ the map $\kappab\mapsto u$, mapping the discretized coefficient
to the numerical solution of equation \ref{eq:elliptic}.
The observation map is defined by the operator
$B_i(u)\coloneqq\int_\Dc u\,\phi_i\,\d\xb$, where
$\phi_i(\xb)\coloneqq\exp[-\Vert\sbb_i-\xb\Vert_2^2/(2\delta^2)]/\gamma_i$,
$\{\sbb_i\}_{i=1}^n\in\Dc$ are observation locations, $\delta=10^{-4}$,
and $\gamma_i$ are normalization constants so that $\int_\Dc \phi_i\,\d\xb=1$ for all $i=1,\ldots,n$.
The parameter-to-observation map is then defined by
$\Fc:\kappab\mapsto [B_1(\Sc(\kappa)), \ldots,B_n(\Sc(\kappa))]^\top$.
The coefficient $\kappa$ is endowed with the distribution
$\kappa\sim\Nc(0,\Cc(\xb,\xb^\prime))$, where
$\Cc(\xb,\xb^\prime)\coloneqq\exp(-\Vert \xb -\xb^\prime\Vert_2)$
is the Ornstein–Uhlenbeck (exponential) covariance kernel.
Letting $\Sigma$ be the discretization of $\Cc$ over the finite element mesh,
we define the likelihood to be
$\Lc_{\yb}(\zb)\propto\exp\left(-\left\Vert \yb - \Fc(\Sigma^{1/2}\zb) \right\Vert_{\Sigma_{\text{obs}}^{-1}}\right)$.
We stress here that the model is computationally demanding:
the evaluation of $\pi(\zb)$ and $\nabla\pi(\zb)$ require approximately
$1$ second.

Figure \ref{fig:app:elliptic} shows the observation generating solution
$u^\star = \Sc(\kappab)$,
the posterior mean $\mathbb{E}[\kappab\vert\yb^\star]$ and the posterior
standard deviation $\operatorname{Std}[\kappab\vert\yb^\star]$.

==> arXiv v2/additional-example-lgcp.tex <==
\subsection{Additional example: Log-Gaussian Cox process with sparse observations}\label{app:examples:log-cox}

We consider an inference problem in
spatial statistics for a log-Gaussian Cox point process on a square domain 
$\mathcal{D} = [0,1]^2$.
This type of stochastic process
is frequently used to model spatially aggregated point patterns % that can arise,
%for instance, due to environmental heterogenity 
\cite{moller1998,Christensen2005,rue2009approximate,girolami2011riemann}.
%
Following a configuration similar to \cite{Christensen2005,moller1998}, we
discretize $\mathcal{D}$ into a $64 \times 64$ uniform grid, and denote by   
%$\Sc=\{ \sbb_1 ,\ldots, \sbb_n \}$, where
$\sbb_i \in \mathcal{D}$  the center of the
$i$th cell, for $i=1,\ldots,d$,  with $d=64^2$.
% and  the set of locations of the
% centers of each cell in the grid,  with $\sbb_i \in \mathcal{D}$ and $n=64^2$.
We consider a discrete stochastic process $(\Yb_i)_{i=1}^d$, where $\Yb_i$ 
denotes the number of occurrences/points in the $i$th cell.
% (For instance, $\Yb_i$ could denote the number of crimes in the
% $i$th neighborhood during a certain period of time.)
Each $\Yb_i$ is modeled as a Poisson random variable with mean 
$\exp( \Zb_i )/d$, where $(\Zb_i)$ is a Gaussian process
with covariance
$\cov(\Zb_i,\Zb_j) = 
\sigma^2 \exp \left( - \left\Vert \sbb_i - \sbb_j \right\Vert_2 /
(64 \beta) \right)$
% %\todo{db:should it be $64\beta$ in the denomiator? See Christiansen}
% \begin{equation}
%   \label{eq:LogGaussianCox:cov}
%   \cov(\Zb_i,\Zb_j) = 
%   \sigma^2 \exp \left( - \frac{\left\Vert \sbb_i - \sbb_j \right\Vert_2}{ \beta } \right) \;,
% \end{equation}
%$\ell = 1.1 \times 10^{-2}$, 
and mean $\Ex[\Zb_i] = \mu$, for all $i=1,\ldots,d$.
% We consider the following values for the parameters:
% $\beta=1/33$, $\sigma^2 = 1.91$, and $\mu = \log(126)-\sigma^2/2$ (see \cite{Christensen2005} for more details).
We consider the following values for the parameters:
$\beta=1/33$, $\sigma^2 = 1.91$, and $\mu = \log(126) - \sigma^2/2$.
%\todo{New correlation length 0.7/64 ?}
The $(\Yb_i)$ are assumed conditionally independent given the (latent) Gaussian field.
For interpretability reasons, we also 
define the {\it intensity} process $(\Lambdab_i)_{i=1}^d$ as $\Lambdab_i = \exp( \Zb_i )$,
for $i=1,\ldots,d$.
%\todo{Intensity process here}
%

The goal of this problem is to infer the posterior distribution of the
latent process $\Lambdab \coloneqq (\Lambdab_1,\ldots,\Lambdab_n)$
% -- or equivalently $\Zb$ -- 
given 
few sparse realizations of
$\Yb\coloneqq(\Yb_i)$ at $n=30$ spatial locations  $\sbb_{k_1},\ldots, \sbb_{k_n}$ shown in
Figure \ref{fig:ex:LogCox:TruthAndRealizations}.
% Thus, we set $\Yb \coloneqq ( \Yb_{k_1},\ldots, \Yb_{k_n} )$ and
We denote by $\yb^\star \in \re^n$ a realization of $\Yb$ obtained by sampling
the latent Gaussian field according to its marginal distribution.
Our target distribution is then:
$\pi_{\Lambdab \vert \Yb}({\bm\lambda} \vert \yb^\star)$.
% $\pi_{\Lambdab \vert \yb^\star}({\bm\lambda}) \coloneqq  \pi_{\Lambdab \vert \Yb}({\bm\lambda} \vert \yb^\star)$.

Since the posterior is nearly Gaussian,
we will run three experiements with linear lazy maps and
ranks $r=1,3,5$.
For the three experiments,
the KL-divergence minimized for each lazy
layer and the estimators of $H^\text{B}_\ell$
are discretized with
$m=100,300,500$ Monte Carlo samples respectively.
% The matrix $H_\rho$ will be approximated using $m=100$
% Monte-Carlo samples from $\rho$.
% The $1,3,5$-dimensional densities
% $\pi^\star$ are approximated by one-sample approximations ($n_\star=1$
% in Algorithm \ref{alg:lazy-map-construction}).



Figures \ref{fig:ex:LogCox:posterior-expectation}--\subref{fig:ex:LogCox:posterior-realizations}
show the expectation and few realizations of the posterior,
confirming the data provides some
valuable information to recover the field $\Lambdab$.
Figures
\ref{fig:ex:LogCox:convergence}--\subref{fig:ex:LogCox:convergence-cost}
show the convergence rate and the cost of the
algorithm as new layers of lazy maps are added to $\frak{T}_\ell$.
As we expect, the use of maps with higher ranks leads to faster
convergence. On the other hand the computational cost per step
increases---also due to the fact that we increase the
sample size $m$ as the rank increases.
Figure \ref{fig:ex:LogCox:spectrum} reveals the spirit of the
algorithm: each lazy map trims away power from the top of the
spectrum of $H$, which slowly flattens \emph{and} decreases.
To additionally confirm the quality of $\frak{T}_6$ for lazy maps with
rank $5$, and to produce asymptotically unbiased samples from $\pi$, we sample the pullback distribution $\frak{T}_6^\sharp \pi$
using an MCMC chain of length $10^4$, with a Metropolis independence
sampler employing a $\mathcal{N}(0,I_d)$  proposal (see [C. Robert and G. Casella, \emph{Monte Carlo statistical methods}, 2013] for more details).
% , with stationary distribution
% $\frak{T}_6^\sharp\pi$, using the independent Metropolis-Hastings
% algorithm \cite{robert2013monte}
% with proposal distribution $\mathcal{N}(0,I_d)$. 
As explained in \cite{parno2014transport}, the Metropolis independence
sampler is effective insofar as the pullback distribution has
been Gaussianized by the map.
The reported
acceptance rate is $72.6\%$ with the worst effective sample size
(over all $d=4096$ chain components) being
$26.6\%$ of the total chain.

\begin{figure}[t]
	\centering
	\begin{subfigure}[b]{.32\linewidth}
		\includegraphics[width=0.9\textwidth]{./lgc-plots/ExpField-Obs.pdf}
		\caption{Field $\Lambdab^\star$ and observations $\yb^\star$}
		\label{fig:ex:LogCox:TruthAndRealizations}
	\end{subfigure}
	\hspace{2pt}
	\begin{subfigure}[b]{.28\linewidth}
		\includegraphics[width=0.86\textwidth]{./lgc-plots/mean-exp-space.pdf}
		\caption{$\mathbb{E}[\Lambdab\vert\yb^\star]$}
		\label{fig:ex:LogCox:posterior-expectation}
	\end{subfigure}
	\hspace{3pt}
	\begin{subfigure}[b]{.32\linewidth}
		% \begin{subfigure}[b]{.48\linewidth}
		\includegraphics[width=.39\textwidth]{./lgc-plots/realization-2-exp-space.pdf}
		% \end{subfigure}
		\hspace{1pt}
		% \begin{subfigure}[b]{.48\linewidth}
		\includegraphics[width=.39\textwidth]{./lgc-plots/realization-4-exp-space.pdf}
		% \end{subfigure}
		\\[2pt]
		% \begin{subfigure}[b]{.48\linewidth}
		\includegraphics[width=.39\textwidth]{./lgc-plots/realization-10-exp-space.pdf}
		% \end{subfigure}
		\hspace{1pt}
		% \begin{subfigure}[b]{.48\linewidth}
		\includegraphics[width=.39\textwidth]{./lgc-plots/realization-16-exp-space.pdf}
		% \end{subfigure}
		\caption{Realizations of $\Lambdab\sim\pi_{\Lambdab\vert\yb^\star}(\lambdab)$}
		\label{fig:ex:LogCox:posterior-realizations}
	\end{subfigure}
	\\[10pt]
	\begin{subfigure}[b]{.32\linewidth}
		\includegraphics[width=\textwidth]{./lgc-plots/convergence-rate.pdf}
		\caption{Convergence rate}
		\label{fig:ex:LogCox:convergence}
	\end{subfigure}
	\begin{subfigure}[b]{.32\linewidth}
		\includegraphics[width=\textwidth]{./lgc-plots/convergence-rate-cost.pdf}
		\caption{Convergence and cost vs. ranks}
		\label{fig:ex:LogCox:convergence-cost}
	\end{subfigure}
	\hspace{2pt}
	\begin{subfigure}[b]{.31\linewidth}
		\includegraphics[width=\textwidth]{./lgc-plots/spectrum-r5-o1-extra.pdf}
		\caption{Spectrum decay}
		\label{fig:ex:LogCox:spectrum}
	\end{subfigure}
	
	% \begin{subfigure}[b]{.30\linewidth}
	%   \includegraphics[width=\textwidth]{./figs/LogGaussianCox/std-exp-space.pdf}
	%   \caption{$\mathrm{Std}[\Lambdab\vert\yb^\star]$}
	%   \label{fig:ex:LogCox:posterior-std}
	% \end{subfigure}
	% % \end{minipage}
	% \hspace{3pt}
	
	\caption{
		Application of the algorithm on the log-Gaussian Cox
		process distribution.
		Figure (\subref{fig:ex:LogCox:TruthAndRealizations}) shows the intensity field
		$\Lambdab^\star$ used to generate the data $\yb^\star$ (circles).
		Figures
		(\subref{fig:ex:LogCox:posterior-expectation}) shows the
		posterior expectation.
		Figure (\subref{fig:ex:LogCox:posterior-realizations}) shows four
		realizations from the posterior $\pi(\Lambdab\vert\yb^\star)$.
		Figure (\subref{fig:ex:LogCox:convergence}) shows the convergence
		rate of the algorithm as a function of the iterations.
		Figure (\subref{fig:ex:LogCox:convergence-cost}) shows the cost of the
		algorithm for different truncation ranks.
		Figure (\subref{fig:ex:LogCox:spectrum}) shows the decay of the
		spectrum of $H_\ell$ for lazy maps with rank $5$.
	}
	\label{fig:ex:LogCox}
\end{figure}

==> arXiv v2/additional-example-timoshenko.tex <==
\subsection{Additional example: Estimation of the Young's modulus of a cantilever beam}
\label{app:examples:timoshenko}


\begin{figure}
	\centering
	\begin{subfigure}[b]{.31\linewidth}
		\includegraphics[width=\textwidth]{./timoshenko-solution-sensors.pdf}
		\caption{Experimental setting}
		\label{fig:ex:cantilever:experiment-setting}
	\end{subfigure}
	\hspace{3pt}
	\begin{subfigure}[b]{.31\linewidth}
		\includegraphics[width=\textwidth]{./timoshenko-convergence.pdf}
		\caption{Convergence rate}
		\label{fig:ex:cantilever:convergence}
	\end{subfigure}
	\hspace{5pt}
	\begin{subfigure}[b]{.28\linewidth}
		\includegraphics[width=\textwidth]{./timoshenko-aligned-marginals.pdf}
		\caption{Marginals of $\pi(\Eb\vert\yb^\star)$}
		\label{fig:ex:cantilever:aligned-marginals}
	\end{subfigure}
	\caption{
		Application of the algorithm for the estimation of the Young's
		modulus of a cantilever beam.
		Figure (\subref{fig:ex:cantilever:experiment-setting}) shows the
		experimental setting with the beam clamped at $x=0$, the load
		applied at $x=l$, $20$ sensors marked in red, and the true Young's
		modulus [$\SI{}{\giga\pascal}$] for each segment.
		Figure (\subref{fig:ex:cantilever:convergence}) shows the
		convergence of the algorithm in terms of the variance and trace diagnostics.
		Figure (\subref{fig:ex:cantilever:aligned-marginals}) shows
		marginals of the posterior distribution $\pi(\Eb\vert\yb^\star)$
		along with the true values (red).
	}
	\label{fig:ex:cantilever}
\end{figure}

Here we consider the problem of estimating the Young's modulus $E(x)$
of an inhomogeneous cantilever beam, i.e., a beam clamped on one side ($x=0$) and
free on the other ($x=l$).
The beam has a length of $l=\SI{10}{\meter}$,
a width of $w=\SI{10}{\centi\meter}$ and
a thickness of $h=\SI{30}{\centi\meter}$.
Using Timoshenko's beam theory, the displacement $u(x)$
of the beam under the load $q(x)$ is modeled by the coupled PDEs
\begin{equation}
\label{eq:ex:timoshenko-pde}
\begin{cases}
\ddx \left[ \frac{E(x)}{2(1+\nu)} \left( \varphi(x) - \ddx w(x) \right) \right] = \frac{q(x)}{\kappa A} \;, \\
\ddx \left( E(x) I \ddx \varphi(x) \right) = \kappa A \frac{E(x)}{2(1+\nu)} \left( \varphi(x) - \ddx w(x) \right) \;,
\end{cases}
\end{equation}
where  $\nu=0.28$ is the Poisson ratio,
$\kappa=5/6$ is the Timoshenko shear coefficient for rectangular
sections, $A=wh$ is the cross-sectional area of the beam, and
$I=wh^3/12$ is its second moment of inertia. We consider a beam composed of $d=5$ segments each of $\SI{2}{\meter}$ length
made of different kinds of steel,
with Young's moduli
$\Eb^\star=\{E_i\}_{i=1}^5 = \{190, 213, 195, 208, \SI{200}{\giga\pascal}\}$ respectively,
and we run the virtual experiment of applying
a point mass of $\SI{5}{\kilo\gram}$ at the tip of the beam.
% This corresponds to setting $q(x) = - \delta_{l}(x) \cdot \SI{49.05}{\newton}$.
Observations $\yb^\star$ of the displacement $w$ are gathered at the
locations shown in Figure
\ref{fig:ex:cantilever:experiment-setting} with a measurement noise of $\SI{1}{\milli\meter}$. 
We endow $\Eb$ with the prior
$\pi(\Eb)=\Nc(\SI{200}{\giga\pascal},25\cdot I_5)$ and
our goal is to characterize the posterior distribution
$\pi(\Eb\vert\yb^\star) \propto \Lc_{\yb^\star}(\Eb)\pi(\Eb)$. Let $\Sc$ be the map $\Eb \mapsto w$ delivering the solution to (\ref{eq:ex:timoshenko-pde}).
Observations are gathered through the operator $B_i(w)\coloneqq\int_0^l w\,\phi_i\,\d\xb$,
where $\phi_i$ are defined the same way as in Appendix \ref{app:examples:elliptic}
for locations $\{s_i \coloneqq i \cdot 0.5\}_{i=1}^{20}$.
Defining the parameter-to-observable map $\Fc:\Eb\mapsto [B_1(\Sc(\Eb)),\ldots,B_{20}(\Sc(\Eb))]^\top$,
observations $\yb$ are assumed to satisfy the model $\yb = \Fc(\Eb) + \epsilon$,
where $\epsilon \sim \Nc(0, 10^{-6} \cdot I_{20})$ corresponds to $\SI{1}{\milli\meter}$
of measurement noise.

The algorithm is run with rank $2$ lazy maps using triangular
polynomial maps  of degree $3$ as the underlying transport class. The
expectations appearing in the algorithms are approximated using $m=100$ samples from $\Nc(0,I_5)$.
Figures \ref{fig:ex:cantilever} and \ref{fig:app:ex:cantilever} summarize the results.
We further confirm these results by generating an MCMC chain of length
$10^4$ using Metropolis-Hastings with a $\mathcal{N}(0,I_d)$
independence proposal; the target distribution for MCMC is the
pullback $\frak{T}_\ell^\sharp\pi$, as in previous examples.
% independent Metropolis-Hastings algorithm \cite{robert2013monte}.
The reported acceptance rate is $68.3\%$
with the worst, best, and
average effective sample sizes being $7.0\%$, $38.7\%$, and $20.1\%$
of the complete chain. 
In this example we fix
the Poisson ratio, but one could think of it varying from material to
material, and thus estimate it jointly with the Young's modulus.


\begin{figure}
	\centering
	\begin{subfigure}[b]{.31\linewidth}
		\includegraphics[width=\textwidth]{./timoshenko-field-distr-vs-synthetic.pdf}
		\caption{True field vs. posterior}
		\label{fig:ex:cantilever:true-vs-posterior}
	\end{subfigure}
	\hspace{3pt}
	\begin{subfigure}[b]{.31\linewidth}
		\includegraphics[width=\textwidth]{./timoshenko-posterior-predictive-obs-mismatch-ratio.pdf}
		\caption{Posterior predictive mismatch}
		\label{fig:ex:cantilever:post-pred}
	\end{subfigure}
	\caption{
		Additional results for the estimation of Young's
		modulus of a cantilever beam.
		Figure (\subref{fig:ex:cantilever:true-vs-posterior}) shows the
		mean (dashed black) and the $5,10,90,95$-percentiles (thin black)
		of the marginals of $\pi(\Eb\vert\yb^\star)$ compared with the true values
		(red).
		Figure (\subref{fig:ex:cantilever:post-pred}) shows the
		distribution of $(\yb^\star - \yb)/\vert\yb^\star\vert$,
		where $\yb$ is distributed
		according to the posterior predictive
		$\pi(\yb\vert\yb^\star)=\pi(\yb\vert \Eb)\pi(\Eb\vert\yb^\star)$.
	}
	\label{fig:app:ex:cantilever}
\end{figure}

==> arXiv v2/broader-impact.tex <==
\section*{Broader Impact}

\paragraph{Who may benefit from this research?}
We believe users and developers of approximate inference methods will benefit from our work.
%
Our framework works as an ``outer wrapper'' that can improve the effectiveness of any flow-based variational inference method by guiding its structure. We hope to make expressive flow-based variational inference more tractable, efficient, and broadly applicable, particularly in high dimensions, by developing automated tests for low-dimensional structure and flexible ways to exploit it.
%
The trace diagnostic developed in our work rigorously assesses the quality of transport/flow-based inference, and may be of independent interest.% depend purely on the quali of the posterior approximation
%Error in approximate inference can manifest in several ways. We note that a common downstream application of inference is to answer questions of the form: is the mean/mode of the posterior distribution sufficiently far from some threshold (typically based on the posterior variance)? Or, is the probability of some undesirable event sufficiently small? These are common paradigms for decision making. A common phenomena of classic variational inference methods is to under-report the variance in the posterior, %  (because they minimize the KL in the exclusive direction). 
%which causes trouble in answering either of the above questions. 
%Our framework works as an ``outer wrapper'' that can improve the effectiveness of any flow-based variational inference method by guiding its structure. We hope to make expressive flow-based variational inference methods more tractable, efficient, and broadly applicable by developing automated tests for low-dimensional structure and flexible ways to exploit it. We also note that the trace diagnostic developed in our work depends purely on the quality of the posterior approximation and can be used for deciding whether approximate posterior summaries are accurate enough to use for some application.
%
%Posterior predictive scores often are not sensitive to such issues. 
%Algorithmically, our lazy framework works as an ``outer wrapper'' that can improve the effectiveness of any flow-based variational inference method by guiding its structure. We hope to make expressive flow-based variational inference methods more tractable for high dimensional problems, efficient, and broadly applicable by developing automated tests for low-dimensional structure and flexible ways to exploit it.
%The diagnostics developed in our work, for rigorously assessing the quality of transport/flow-based inference, depend purely on the quality of the posterior approximation
%%and help control the inclusive KL divergence
%. This \todo{The antecedent of `this' is a little fuzzy. This feature, this [something]\ldots?} is essential for deciding whether approximate posterior summaries are accurate enough to use for some application.

%The diagnostics developed in our work depend purely on the quality of the posterior approximation and can be used for deciding whether approximate posterior summaries are accurate enough to use for some application.
%and help control the inclusive KL divergence
%. This \todo{The antecedent of `this' is a little fuzzy. This feature, this [something]\ldots?} is essential for deciding whether approximate posterior summaries are accurate enough to use for some application.

%Algorithmically, our lazy framework works as an ``outer wrapper'' that can improve the effectiveness of any flow-based variational inference method by guiding its structure. We hope to make expressive flow-based variational inference methods more tractable, efficient, and broadly applicable by developing automated tests for low-dimensional structure and flexible ways to exploit it.


 % and we note it theoretical underpinning works to control the inclusive KL divergence. Also, the diagnostics developed in this work, for assessing the quality of transport/flow-based inference, depend purely on the quality of the posterior approximation, which is valuable for deciding if the approximate posterior summaries are accurate enough to use for some application.



% \todo{Add something here about making expressive flow-based variational inference more tractable, by developing automated tests and diagnostics for low-dimensional structure and generally applicable ways to exploit it. Indeed, we view our lazy framework as an outer wrapper that can improve the effectiveness of any flow-based variational inference method, by guiding its structure.}


\paragraph{Who may be put at disadvantage from this research?}
We don't believe anyone is put at disadvantage due to this research.

\paragraph{What are the consequences of failure of the system?}
We specifically point out that one contribution of this work is identifying when a poor posterior approximation has occurred. A potential failure mode of our framework would be inaccurate estimation of the diagnostic matrix $H$ or its spectrum, suggesting that the approximate posterior is more accurate than it truly is. However, computing the eigenvalues or trace of a symmetric matrix, even one estimated from samples, is a well studied problem. And numerical software guards against poor eigenvalue estimation or at least warns if this occurs. We believe the theoretical underpinnings of this work make it robust to undetected failure. 

\paragraph{Does the task/method leverage biases in the data?}
We don't believe our method leverages data bias. As a method for variational inference, our goal is to accurately approximate a posterior distribution. It is very possible to encode biases for/against a particular result in a Bayesian inference problem, but that occurs at the level of modeling (choosing the prior, defining the likelihood) and collecting data, not at the level of approximating the posterior.
	

==> arXiv v2/conclusions.tex <==
\section{Conclusions}
We have presented a framework for creating target-informed architectures for transport-based variational inference.
%
Our approach uses a rigorous error bound to identify low-dimensional structure in the target distribution and focus the expressiveness of the transport map or flow on an important subspace.
%
% OLD: By solving a particular eigenvalue problem, we are able to identify low dimensional structure in the target distribution, and focus the expressiveness of the transport map on a particular important subspace.
%
We also introduce and analyze a greedy algorithm for building deep compositions of low-dimensional maps that can iteratively approximate general high-dimensional target distributions. Empirically, these methods improve the accuracy of inference, accelerate training, and control the complexity of flows to improve tractability. Ongoing work will consider constructive tests for further varieties of underlying structure in inference problems, and their implications on the structure of flows.

% old:
%We have presented a framework for target-informed architectures 
%% that improve
%for 
%inference with flow/transport methods in high dimensions, using rigorous error bounds 
%% to identify important coordinates 
%to guide the choice of basis
%and achieve dimension reduction. We also introduce and analyze a greedy algorithm for building deep compositions of low-dimensional maps. Empirically, these methods improve the accuracy of inference, accelerate training, and control the complexity of flows to improve tractability. Ongoing work will consider constructive tests for further varieties of underlying structure in inference problems, and their implications on the structure of flows.


% Here we presented a new framework for solving high-dimensional Bayesian inference problems using any class of transport. Our contributions include a principled method for picking a coordinate basis for a transport map, theoretical insights that lead to systematic dimension reduction, and the development of a greedy algorithm for building deep compositions of structure exploiting maps.

% We empirically demonstrated the benefits of our framework on a range of inference, and showed its potential for improving performance metrics, accelerating the training process of the map, and controlling the number of map parameter trained at one time.

% As future work, this framework has inspired us to consider other types underlying structure inference problems, that might yield additional computational benefits and theoretical insights.



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> arXiv v2/dimension-reduction.tex <==
\section{Lazy maps} \label{sec:LazyMaps}
Given a unitary matrix $U\in\R^{d\times d}$ and an integer $r\leq d$,
let $\mathcal{T}_r(U)$ be the set that contains all the maps
$T:\R^d\rightarrow \R^d$ of the form %\todo{blue added to parallel comment in intro $T(x)$ vs $UT(x)$. YMM: great}
\begin{equation}\label{eq:LazyMap}
 T(z)  =  U \left[\begin{array}{c}
 \tau( z_1,\hdots,z_r) \\
 z_\perp
 \end{array}\right] = 
 U_r \tau( z_1,\hdots,z_r) + U_\perp z_\perp
\end{equation}
for some diffeomorphism $\tau:\R^r\rightarrow\R^r$. Here $U_r\in\R^{d\times r}$ and $U_\perp\in\R^{d\times (d-r)}$ are the matrices containing respectively the $r$ first and the $d-r$ last columns of $U$, and $z_\perp=(z_{r+1},\hdots,z_d)$.
% 
Any map $T\in\mathcal{T}_r(U)$ is called a \emph{lazy map} with rank bounded by $r$, as it is nonlinear only with respect to the first $r$ input variables $z_1,\hdots,z_r$ and the nonlinearity is contained in the low-dimensional subspace $\text{range}(U_r)$. 
The next proposition gives a characterization of all the densities $T_\sharp\rho$ when $T\in\mathcal{T}_r(U)$.

\begin{proposition}[Characterization of lazy maps]\label{prop:CaracterizationOfLazyMaps}
 Let $U\in\R^{d\times d}$ be a unitary matrix and let $r\leq d$. 
 Then for any lazy map $T\in\mathcal{T}_r(U)$, there exists a strictly positive function $f:\R^r\rightarrow\R_{>0}$ such that
 \begin{equation}\label{eq:LazyMap_VS_Ridge}
  T_\sharp\rho (x) = f(U_r^\top x)\rho(x),
 \end{equation}
 for all $x\in\R^d$ where $\rho$ is the density of the standard normal distribution.
 Conversely, any probability density function of the form $f(U_r^\top x)\rho(x)$ admits a representation as in \eqref{eq:LazyMap_VS_Ridge} for some $T\in\mathcal{T}_r(U)$.
\end{proposition}
The proof is given in Appendix \ref{proof:CaracterizationOfLazyMaps}.
By Proposition \ref{prop:CaracterizationOfLazyMaps}, any posterior density $\pi(x)\propto\mathcal{L}_y(x)\pi_0(x)$ with standard Gaussian prior $\pi_0=\rho$ and with likelihood function given by $\mathcal{L}_y(x) \propto f(U_r^\top x)$ can be writen \emph{exactly} as $\pi=T_\sharp\rho$ for some lazy map $T\in\mathcal{T}_r(U)$.
% 
% In particular, applying Proposition \ref{prop:CaracterizationOfLazyMaps} to the posterior density $\pi$ introduced in \S\ref{sec:intro}:
% % \eqref{eq:PosteriorDensity}: 
% if the prior distribution is $\pi_0=\rho$ and if the likelihood function is of the form of $\mathcal{L}_y(x) \propto f(U_r^\top x)$, then there exists a lazy map $T\in\mathcal{T}_r(U)$ that exactly recovers the posterior density $T_\sharp\rho=\pi$. 
% 
In particular, posteriors of generalized linear models naturally fall into this class; see Appendix \ref{app:glms} for more details. % \todo{Here is where we could easily refer to GLMs: ``Generalized linear models naturaly fall into this class, as we show in Appendix blah.'' or something like that. MB: How is this? YM: great.}
Following \cite[Section 2.1]{zahm2018certified}, the solution $T^\star\in\mathcal{T}_r(U)$  to
$$
  \Dkl( \pi || T^\star_\sharp\rho) = \min_{T \in \mathcal{T}_r(U)} \Dkl( \pi || T_\sharp\rho),
$$
is such that $T^\star_\sharp\rho(x)
=  f^\star(U_r^\top x) \rho(x) $, where $f^\star$ is the
conditional expectation %\todo{line break}
$$f^\star(x_r)=\Ex \left [ \frac{\pi(X)}{\rho(X)} \vert U_r^\top X=x_r  \right ] $$
with $X\sim\rho$. 
% 
% Following \cite[Section 2.1]{zahm2018certified}, the KL divergence $\Dkl( \pi || T_\sharp\rho)=\Ex_\pi[\log(\pi/T_\sharp\rho)]$ decomposes as
% \begin{equation}\label{eq:PythagoreanKL}
%  \Dkl( \pi || T_\sharp\rho) = \Dkl( \pi || T^\star_\sharp\rho) + \Dkl( T^\star_\sharp\rho || T_\sharp\rho), 
% \end{equation}
% % where $T^\star\in\mathcal{T}_r(U)$ is the minimizer of $\Dkl( \pi || T_\sharp\rho)$ over $T\in\mathcal{T}_r(U)$ for a given $U$ and $r$. This optimal lazy maps writes $T^\star_\sharp\rho(x) =  f^\star(U_r^\top x) \rho(x) $ where $f^\star$ is the conditional expectation $f^\star(x_r)=\Ex [\frac{\pi(X)}{\rho(X)}|U_r^\top X=x_r ]$ with $X\sim\rho$. 
% % 
% % 
% where $T^\star\in\mathcal{T}_r(U)$ is such that $T^\star_\sharp\rho(x)
% =  f^\star(U_r^\top x) \rho(x) $, where $f^\star$ is the
% conditional expectation
% $f^\star(x_r)=\Ex [\frac{\pi(X)}{\rho(X)}|U_r^\top X=x_r ]$
% with $X\sim\rho$. 
% Because $\Dkl( T^\star_\sharp\rho || T_\sharp\rho)\geq0$,
% Equation \eqref{eq:PythagoreanKL} implies $\Dkl( \pi || T_\sharp\rho) \geq \Dkl( \pi || T^\star_\sharp\rho)$ which shows that $T^\star$ is a minimizer of $\Dkl( \pi || T_\sharp\rho)$ over $T\in\mathcal{T}_r(U)$.

Now that we know the optimal lazy map in $\mathcal{T}_r(U)$, it remains to find a suitable matrix $U$ and rank $r$.
% 
% Following \cite{huber1985projection}, we have
In Appendix \ref{proof:KL_Tstar_Decomp} we show that 
\begin{equation}\label{eq:KL_Tstar_Decomp}
 \Dkl( \pi || T^\star_\sharp\rho)
%  = \int \log\left(\frac{\pi(x)}{f^\star(U_r^\top x)\rho(x)} \right)\d\pi \d x
 = \Dkl( \pi || \rho) - \Dkl( (U_r^\top)_\sharp \pi_r || \rho_r ) ,
\end{equation}
where $\rho_r$ is the density of the standard normal distribution on $\R^r$ and $(U_r^\top)_\sharp \pi$ is the density of $U_r^\top X$ with $X\sim\pi$.
%the marginal density of $\pi$ with respect to $U_r$, meaning the density of $U_r^\top X$ with $X\sim\pi$. 
Thus, for fixed $r$, minimizing $\Dkl(\pi||T^\star_\sharp\rho)$ over $U$ is the same as finding the most non-Gaussian marginal $(U_r^\top)_\sharp \pi$. Such an optimal $U$ can be difficult to find in practice. The next proposition instead gives a computable \emph{bound} on $\Dkl( \pi || T^\star_\sharp \rho)$, which we will use to construct a $U$ suitable for our algorithm. 
% that rigorously controls the error in the KL divergence. 
The proof is given in Appendix \ref{proof:LogSobResult}.

\begin{proposition}\label{prop:LogSobResult}
  Let $(\lambda_i,u_i)\in\R_{\geq0}\times\R^d$ be the $i$-th eigenpair of the eigenvalue problem $Hu_i = \lambda_i u_i$ where $H = \int (\nabla\log\frac{\pi}{\rho} )(\nabla\log\frac{\pi}{\rho} )^\top\d\pi$. Let $U=[u_1,\hdots,u_d]\in\R^{d\times d}$ be the matrix containing the eigenvectors of $H$. Then for any $r\leq d$ we have
 \begin{equation}\label{eq:LogSobResult}
  \Dkl( \pi || T^\star_\sharp \rho) \leq \frac{1}{2} (\lambda_{r+1}+\hdots+\lambda_d).
 \end{equation}
\end{proposition}

Proposition \ref{prop:LogSobResult} suggests constructing $U$ as the matrix of eigenvectors of $H$, 
%= \int (\nabla\log\frac{\pi}{\rho} )(\nabla\log\frac{\pi}{\rho} )^\top\d\pi$, \todo{minor, but to save space we could avoid re-quoting the def of $H$ here}
and that a fast decay in the spectrum of $H$ allows a lazy map with low $r$ to accurately represent the true posterior. 
%Indeed, given a sufficiently expressive transport class, one can guarantee existence of a map satisfying $\Dkl( \pi || T_\sharp \rho) < \varepsilon$ by choosing $r$ to be the smallest integer such that the left-hand side of \eqref{eq:LogSobResult} is below $\varepsilon$. 
Indeed, one can guarantee $\Dkl( \pi || T^\star_\sharp \rho) < \varepsilon$ by choosing $r$ to be the smallest integer such that the left-hand side of \eqref{eq:LogSobResult} is below $\varepsilon$.
% \todo{Potentially simpler: Indeed, one can guarantee $\Dkl( \pi || T^\star_\sharp \rho) < \varepsilon$ by choosing \ldots}
%We point out in Appendix \ref{app:glms} that inference problems from generalized linear models ({\bf wording}) admit lazy structure depending on the rank of the matrix of observations. 
In practice, 
%however, the spectrum of $H$ may not decay so that the necessary $r$ is much smaller than the dimension.
since the complexity of representing and training a transport map may strongly depend on $r$, we can bound $r$ by some $r_{{\text{max}}} \leq d$ associated with a computational budget for constructing $T$.
% the maximal computational budget one can afford in constructing $T$. 
% This yields
% \begin{equation}\label{eq:boundRank}
%  r= r_{{\text{max}}} \wedge \min \left\{ r\leq d ~: \frac{1}{2}\sum_{i=r+1}^d\lambda_{i} \leq \varepsilon \right\}.
% \end{equation}
This procedure is summarized in Algorithm \ref{alg:LazyMap}.
% \todo{This may be a good place where to reference the projected SVN work}

%\begin{algorithm}
%  \caption{
%    Construction of a lazy map.
%  }
%  \begin{algorithmic}[1]
%    \Procedure{LazyMap}{$\pi$, $\rho$, $\varepsilon$, $r_{{\text{max}}}$}
%    \State Compute \label{alg:LazyMap:H}
%    $H=\int (\nabla\log\frac{\pi}{\rho} )(\nabla\log\frac{\pi}{\rho} )^\top\d\pi$ 
%%     $$H=\int \left(\nabla\log\frac{\pi}{\rho} \right)\left(\nabla\log\frac{\pi}{\rho} \right)^\top\d\pi$$ 
%    \State Solve the eigenvalue problem $Hu_i=\lambda_iu_i$ 
%    \State Let $r= r_{{\text{max}}} \wedge \min \{ r\leq d ~: \frac{1}{2}\sum_{i>r}\lambda_{i} \leq \varepsilon \}$ and assemble $U=[u_1,\hdots,u_d]$.    
%    \State Find $T$ by solving \label{alg:LazyMap:min} 
%    $\min_{T\in\mathcal{T}_r(U)}\Dkl(T_\sharp\rho||\pi)$
%%     $$\min_{T\in\mathcal{T}_r(U)}\Dkl(\pi||T_\sharp\rho)$$
%    \State\Return lazy map $T$
%    \EndProcedure
%  \end{algorithmic}\label{alg:LazyMap}
%\end{algorithm}

The practical implementation of Algorithm \ref{alg:LazyMap} relies on the computation of $H$. % (step \ref{alg:LazyMap:H}).
%and minimizing the KL divergence (step \ref{alg:LazyMap:min}).
Direct Monte Carlo estimation of $H$, however, requires generating samples from $\pi$, which is not feasible in practice.
% 
%Following \cite{zahm2018certified}, one could use the importance sampling estimate $\widetilde{H} = \frac{1}{K}\sum_{k=1}^K \omega_k (\nabla\log\frac{\pi}{\rho}(X_k))(\nabla\log\frac{\pi}{\rho}(X_k))^\top$, where $X_1,\hdots,X_K$ are i.i.d.\ samples from $\rho$ and where $\omega_k = \frac{\pi(X_k)}{\rho(X_k)}/(\sum_{k'=1}^K \frac{\pi(X_{k'})}{\rho(X_{k'})})$ are self-normalized weights.
% Following \cite{zahm2018certified},
Instead one can use an importance sampling estimate, taking $$H \approx \frac{1}{K}\sum_{k=1}^K \omega_k (\nabla\log\frac{\pi}{\rho}(X_k))(\nabla\log\frac{\pi}{\rho}(X_k))^\top,$$ where $\{X_k\}_{k=1}^K$ are i.i.d.\ samples from $\rho$ and $\omega_k = \frac{\pi(X_k)}{\rho(X_k)}/(\sum_{k'=1}^K \frac{\pi(X_{k'})}{\rho(X_{k'})})$ are self-normalized weights.
%
This estimate can have significant variance when $\rho$ is a poor approximation to the target $\pi$ (e.g., in the first stage of the greedy algorithm in \S\ref{sec:LayersLazyMaps}). In this case it is preferable to impose $\omega_k=1$, which reduces variance but yields an biased estimator of $H$; instead, it is an unbiased estimator of $H^{\text{B}} = \int (\nabla\log\frac{\pi}{\rho} )(\nabla\log\frac{\pi}{\rho} )^\top\d\rho$. As shown via the error bounds in \cite[Sec.\ 3.3.2]{zahm2018certified} this matrix still provides useful information regarding the construction of $U$. We consider the differences between the two estimators in Appendix~\ref{app:biasofH}.
%	
Also, since the effective sample size (ESS) of the importance sampling estimate can be computed with little extra cost after collecting samples, one can use this ESS to choose whether to use $H$ or $H^{\text{B}}$. %\todo{ALT: ``whether to use importance sampling or uniform weights.''}
%	
Other variance reduction methods may also be applicable. For example, simplifications or approximations to the expected outer product of score functions yield natural candidates for control variates.

 % and in the numerical example in Section \ref{sec:NumericalExamples}, such an estimate still provides relevant information regarding the construction of $U$. We also study the behavior of the importance sampled estimate $\widetilde{H}$ and the biased estimate $\widetilde{H}_\rho$ numerically in Appendix \ref{app:biasofH}. 

 % even for small sample size $K$\todo{maybe remove the remark on the sample size...}.

%At step \ref{alg:LazyMap:min} of Algorithm \ref{alg:LazyMap}, we need
In constructing a lazy map $T$ of the form \eqref{eq:LazyMap}, one needs to identify a map $\tau:\R^r \to \R^r$ such that $T_\sharp\rho$ approximates the posterior. One can use any transport class to parameterize $\tau$; Appendices
\ref{app:triangular-maps} and \ref{app:iafmaps} detail the particular maps used in our numerical experiments.
%
% Following the ideas in \cite{transportmaps,bigoni2016nips,spantini2018inference,Jaini2019,Kingma2016}, we seek $\tau$ in a parametric family of \emph{monotone triangular} maps. 
%
%As noted in \cite{spantini2018inference}, minimizing
%$\Dkl(\pi||T_\sharp\rho)$ over this class of parametric
%maps can be challenging because it is difficult to build
%estimators for $\Dkl(\pi||T_\sharp\rho)$ when we cannot sample directly
%from $\pi$.
%
In our setting we can only evaluate $\pi$ up to a normalizing constant, and thus it is expedient to minimize the reverse KL divergence
$\Dkl(T_\sharp\rho||\pi) = \Dkl(\rho||T^\sharp\pi)$, as is typical in variational Bayesian methods---which can be achieved by maximizing a Monte Carlo or quadrature approximation of $\Ex_\rho \left [\log T^\sharp \pi \right ]$. This is equivalent to maximizing the evidence lower bound (ELBO) and using the  {reparameterization trick} \cite{kingma2015reparam} to write the expectation over the base distribution $\rho$. 
% \todo{Michael, can you double-check that these are indeed equivalent? Taking advantage of the invertibility of $T$, my simple algebra shows that we are solving $\max_T \Ex_\rho [ \log \mathcal{L}_y \circ T + \log \rho \circ T + \log \det \nabla T ]$. Note also notational overload for $\mathcal{L}$, which is defined as likelihood earlier. MB: look good to me!}
% \[
% \sfL_T = \Ex_{T_\sharp \rho} \left[ \log p(y|x) \right] - \Dkl(T_\sharp \rho ||\pi).
% \]
% It can be shown that the negative ELBO is a constant shift from the KL divergence in the reversed direction. The gradient of ELBO is commonly computed using the {\it reparameterization trick} \cite{kingma2015reparam}, which expresses the expectation over the base distribution $\rho$. 
% %
Details on the numerical implementation of Algorithm \ref{alg:LazyMap} are given in Appendix \ref{app:numerical-algorithms}. We note that the lazy framework works to control the KL divergence in the inclusive direction, while optimizing the ELBO minimizes the KL divergence in the exclusive direction. We show empirically that this computational strategy provides performance improvements in both directions of the KL divergence between the true and approximate posterior, compared to a baseline that does not utilize the lazy framework. %\todo{Reviewer brought up disconnect (forward vs reverse KL) - but idk how we could address more deeply than this. YMM: agreed, I think this is optimal as is.}

\begin{algorithm}
	\caption{
		Construction of a lazy map.
	}
	\begin{algorithmic}[1]
		\Procedure{LazyMap}{$\pi$, $\rho$, $\varepsilon$, $r_{{\text{max}}}$}
		\State Compute \label{alg:LazyMap:H}
		$H=\int (\nabla\log\frac{\pi}{\rho} )(\nabla\log\frac{\pi}{\rho} )^\top\d\pi$ 
		%     $$H=\int \left(\nabla\log\frac{\pi}{\rho} \right)\left(\nabla\log\frac{\pi}{\rho} \right)^\top\d\pi$$ 
		\State Solve the eigenvalue problem $Hu_i=\lambda_iu_i$ 
		\State Let $r= r_{{\text{max}}} \wedge \min \{ r\leq d ~: \frac{1}{2}\sum_{i>r}\lambda_{i} \leq \varepsilon \}$ and assemble $U=[u_1,\hdots,u_d]$.    
		\State Find $T$ by solving \label{alg:LazyMap:min} 
		$\min_{T\in\mathcal{T}_r(U)}\Dkl(T_\sharp\rho||\pi)$
		%     $$\min_{T\in\mathcal{T}_r(U)}\Dkl(\pi||T_\sharp\rho)$$
		\State\Return lazy map $T$
		\EndProcedure
	\end{algorithmic}\label{alg:LazyMap}
\end{algorithm}
% Indeed, the relation
% $
%   \Dkl(T_\sharp\rho||\pi) = \Dkl(\rho||T^\sharp\pi) = \int \log(\rho(x))\rho(x)\d x -\int\log(T^\sharp\pi)\rho(x)\d x
% $
% holds and show that the minimizer of $\Dkl(T_\sharp\rho||\pi)$ is the same as the maximizer of $\int\log(T^\sharp\pi)\rho(x)\d x$. The integral in this last quantity

% Let us insist on the fact that, in general, approximation in the
% reversed KL direction is not the same as in the direct direction, so
% that we have no theoretical guarantee that $T$ will goes to
% $T^\star$.\todo{db: this sentence is a little too apologetic. Could be
% removed.}
% However we show numerically that this computationally feasible strategy yields very good results.


% A change of variable $x=T(z)$ allows to write
% \begin{align*}
%  \Dkl( T_{\sharp}\rho || \pi) 
%  = \Dkl( \rho || T^{\sharp}\pi) 
% %  = \int\log\left( \frac{\rho(x)}{T_{\sharp}\pi(x)}\right) \rho(x) \d x 
%  = \int\log(\rho(z)) \rho(z) \d z - \int\log (T^{\sharp}\pi(z)) \rho(z) \d z ,
% \end{align*}
% so that minimizing $T\mapsto\Dkl( T^{\sharp}\rho || \pi)$ is the same as maximizing $T\mapsto\int\log (T^{\sharp}\pi ) \d\rho$. Here $T^{\sharp}\pi$ denotes the pullback density of $\pi$ through $T$, that is the density of $T^{-1}(X), X\sim\pi$.
% As we will see later on, a Monte Carlo approximation of $\int\log (T^{\sharp}\pi ) \d\rho$ can be obtained using samples from the reference density $\rho$ and not from the target $\pi$.
% % 
% This nice property is no longer true when we switch the arguments in the KL divergence \eqref{eq:KLDivergence}. 


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> arXiv v2/intro.tex <==
\section{Introduction}
\label{sec:intro}
% Inference in the Bayesian setting typically requires the computation of integrals $\int f({x}) \pi({x}) \d{x}$, where $\pi$
% %
% is the density\footnote{In this paper, we only consider distributions that are absolutely
%   continuous with respect to the Lebesgue measure on $\mathbb{R}^d$, and thus
%   will use the notation $\pi$ to denote both the distribution and
%   its associated density.}  
% of some analytically \textit{intractable} (posterior) distribution which is known up to a normalizing constant.
Inference in the Bayesian setting typically requires the computation of integrals $\int f  \, \d\pi$  over an \textit{intractable} posterior distribution whose density\footnote{In this paper, we only consider distributions that are absolutely continuous with respect to the Lebesgue measure on $\mathbb{R}^d$, and thus will use the notation $\pi$ to denote both the distribution and its associated density.} $\pi$ is known up to a normalizing constant.
%
One approach to this problem is to construct a
deterministic nonlinear transformation, i.e., a \emph{transport map}
\cite{villani2008optimal},
%, also referred to as a normalizing flow (see \cite{papamakarios2019normalizing,otherNFreview} for an overview), 
that induces a coupling of $\pi$ with a tractable distribution
$\rho$ (e.g., a standard Gaussian).
Formally, we seek a map $T$ that pushes forward $\rho$ to $\pi$, written as $T_\sharp \rho = \pi$, such that the change of variables
$\int f \, \d \pi = \int f \circ T \, \d \rho $ makes integration
tractable.

Many constructions for such maps have been developed in recent years. Normalizing flows (see \cite{rezende2015variational,tabak2013family,papamakarios2019normalizing,kobyzev2020normalizing} and references therein) build transport maps via a deep composition of functions parameterized by neural networks, 
with certain ansatzes 
% while enforcing certain structure
 to enable efficient computation. Many recently proposed autoregressive flows (for example \cite{dinh2016density,Kingma2016,papamakarios2017masked,huang2018neural,de2019block}) compose triangular maps, which allow for efficient evaluation of Jacobian determinants. In general, triangular maps \cite{bogachev2005triangular,rosenblatt1952remarks,knothe1957contributions} are
sufficiently general to couple any absolutely continuous pair of
distributions $(\rho, \pi)$, and their numerical approximations have
been investigated in \cite{el2012bayesian,marzouk2016introduction, spantini2018inference, Jaini2019}. The flow map of a neural ordinary differential equation \cite{Chen2018,Dupont2019,gholaminejad2019anode} can also be seen as an infinite-layer limit of a normalizing flow. Alternatively, Stein variational methods \cite{liu2016stein,liu2017stein,Detommaso2018} provide a nonparametric way of constructing $T$ as a composition of functions lying in a chosen RKHS.

In general, it can be difficult to represent expressive maps in high dimensions. For example, triangular maps on $\mathbb{R}^d$ must describe $d$-variate functions and thus immediately encounter the curse of dimensionality. Similarly, kernel-based methods lose expressiveness in high dimensions \cite{Detommaso2018,Chen2019}. Flow-based methods often increase expressiveness by adding layers, but this is typically performed in an ad hoc or unstructured way, which also requires tuning. 

Here we propose a framework for inference that creates target-informed architectures around \emph{any} class of transport maps or normalizing flows. In particular, our framework uses rigorous \textit{a priori} error bounds to discover and exploit low-dimensional structure in a given target distribution. It also provides a methodology for efficiently solving high-dimensional inference problems via greedily constructed compositions of \emph{structured} low-dimensional maps. 

The impact of our approach rests on two observations. 
%
First, the coordinate basis in which one expresses a transport map (i.e., $T(x)$ versus $U T(x)$, where $U$ is a rotation on $\R^d$) can 
% drastically change
strongly affect
% \todo{pretty strong there. OK, or should we say ``significantly affect'' ``strongly affect''}
 the training behavior and final performance of the method. Our framework identifies an ordered basis that best reveals a certain low-dimensional structure in the problem. Expressing the transport map in this basis focuses the expressiveness of the underlying transport class and allows for principled dimension reduction. This basis is identified by minimizing an upper bound on the Kullback--Leibler (KL) divergence between $\pi$ and its approximation, which follows from logarithmic Sobolev inequalities (see \cite{zahm2018certified}) relating the KL divergence to gradients of the target density. % via an {average derivative functional} \cite{samarov1993exploring}.

% mention GREEDY
Second, in the spirit of normalizing flows, we seek to increase the expressiveness of a transport map using repeated compositions. Rather than specifying the length of the flow before training, we increase the length of the flow sequentially. For each layer, we apply the framework above to a \emph{residual} distribution that captures the deviation between the target distribution and its current approximation. We prove weak convergence of this greedy approach to the target distribution under reasonable assumptions. This sequential framework enables efficient layer-wise training of high-dimensional maps, which especially helps control the curse of dimensionality in certain transport classes. As we shall demonstrate empirically, the greedy composition approach can further improve accuracy at the end of training, compared to baseline methods. 




%({\bf I think I capture this section above, except for information on where the bound comes from. I dont think that is needed here.})
% We considers maps are low-dimensional in
%that the transformation is restricted to a low-dimensional subspace of the
%parameter space; thus they are termed ``lazy.'' We identify the low-dimensional subspaces sequentially, by greedily minimizing a bound on the KL divergence between $\pi$ and its approximation. The bound itself follows from
%logarithmic Sobolev inequalites (see \cite{zahm2018certified})
%relating the KL divergence to gradients of the target density. We
%prove weak convergence of this approach to the target distribution,
%given even suboptimal choices of the subspace.
%
%


%{\bf I'm not sure if we need to this, it seems out of context in the intro (they don't know what low dimensional structure is yet) -->}
%We point out that while the lazy framework is able to identify and efficient capture exact low dimensional structure in a problem, the overall approach does not require the problem to be specifically structured. We also emphasize that our overall approach does not require any \emph{global} low dimensionality in the likelihood function (as in \cite{cui2014likelihood,Chen2019}, for example).%: rather, it can converge even for maps that act on a single direction at a time, despite $\pi$ and $\rho$ differing in all directions.

% despite the difference between $\pi$ and $\rho$ not being confined to a low-dimensional subspace. 


% \section{Preliminaries}

Since Markov chain Monte Carlo (MCMC) methods are also a workhorse of inference, it is useful to contrast them with the variational methods discussed above. In general, these two classes of methods have different computational patterns. In variational inference, one might spend considerable effort to construct the approximate posterior, but afterwards enjoys cheap access to samples and normalized evaluations of the (approximate) target density. How well the approximation matches the true posterior depends on the expressiveness of the approximation class and on one's ability to optimize within this class. 
%---two qualities our proposed framework seems to improve. 
MCMC, in contrast, requires continual computational effort (even after tuning), but (asymptotically) generates samples from the exact posterior. Yet there is a line of work that uses transport to improve the performance of MCMC methods (\cite{parno2014transport,hoffman2019neutra})---such that even if one desires exact samples, constructing a transport map can be beneficial. We will demonstrate this link in our numerical experiments.



% FROM REBUTTAL
% Finding a fair comparison between MCMC and VI is a universal and interesting question in Bayesian computation, as the two methods have different computational cost patterns. In VI one spends considerable computational effort to construct the approximate posterior, but afterwards has cheap access to (approximate) samples and normalized density evaluations. How well the approximation matches the true posterior depends on the expressiveness of the transport map/flow and the ability to optimize the map---two qualities that the lazy map framework seems to improve. MCMC methods in contrast require continual computational effort (even after tuning), but (asymptotically) generate samples from the exact posterior.  We will discuss these trade-offs to additionally frame our contribution in the final paper. The strongest comparison we believe we can make is comparing the ESS of an MCMC method with and without transport preconditioning (as discussed in [23, 41] and in \S4.4). We will make these improvements a more central measure of success and will also report the improvements when applied to the examples of \S4.2 and \S4.3.


\paragraph{Preliminaries.} We will consider target distributions with densities $\pi$ on $\mathbb{R}^d$ that are differentiable almost everywhere and that can be evaluated up to a normalizing constant. Such a target will often be the posterior of a Bayesian inference problem, e.g., % \todo{Could inline Bayes rule}
% \begin{equation}\label{eq:PosteriorDensity}
$
 \pi(x) \coloneqq p(x\vert y) \propto \mathcal{L}_y(x) \pi_0(x),
$
% \end{equation}
where $\mathcal{L}_y(x) \coloneqq p(y \vert x)$ is the likelihood function and $\pi_0$ is the prior. We denote the standard Gaussian density on $\mathbb{R}^d$ as $\rho$. We will consider maps $T: \mathbb{R}^d \to \mathbb{R}^d$ that are diffeomorphisms,\footnote{In general $T$ does not need to be a diffeomorphism, but only a
  particular invertible map; see Appendix \ref{app:triangular-maps}
  for more details. The distributions we will consider in this paper, however, fulfill the necessary
  conditions for $T$ to be differentiable almost everywhere.}
and with some abuse of notation, we will write the pushforward density of $\rho$ under $T$ as $T_\sharp\rho(x) \coloneqq \rho \circ T^{-1}(x) \vert \nabla T^{-1}(x) \vert$. We will frequently also use the notion of a \emph{pullback} distribution or density, written as $T^\sharp\pi \coloneqq (T^{-1})_\sharp\pi$.

%{\bf Before:}
%Our goal is to find a map $T$ that satisfies  $\Dkl( \pi || T_{\sharp}\rho ) \leq \varepsilon$ for some prescribed tolerance $\varepsilon > 0$. In Section \ref{sec:LazyMaps} we show how to build a single map in the ``lazy'' format described above. However, the map complexity needed to satisfy the prescribed tolerance might be large if $\varepsilon$ is too small. We thus show in Section \ref{sec:LayersLazyMaps} how to improve our approximations by greedily composing many lazy maps.

In \S\ref{sec:LazyMaps} we show how to build a single map in the low-dimensional ``lazy'' format described above, and describe the class of posterior distributions that admit such structure. In \S\ref{sec:LayersLazyMaps} we develop a greedy algorithm for building deep compositions of lazy maps, which effectively decomposes any inference problem into a series of lower-dimensional problems. %\todo{Reviewer: approximate vs decomposes. I say we stick to decomposes. Its not the decomposition that is approximate, its the limitation of the underlying class of maps. YMM: agreed!}
% Each layer of such a map is constructed to transform the base distribution along a subspace we learn to be most important to improving the performance of the map. 
\S\ref{sec:NumericalExamples} presents numerical experiments highlighting the benefits of the lazy framework.
%
While our numerical experiments employ inverse autoregressive flows \cite{Kingma2016} and polynomial transport maps \cite{Jaini2019,el2012bayesian} as the underlying transport classes, we emphasize that the lazy framework is applicable to any class of transport. 
% The complexity of the map, and hence the computational effort, can be tailored at each layer, making the method exceptionally flexible. 
%\todo{Possibly omit one or two last sentences. MB: agreed for last one (we make that point later anyway) I think we keep the point about other classes as a guard against 'you didn't implement our favorite flow I think would have worked better'}


%% REVISED STUFF ABOVE
% %% OLD STUFF (source material) BELOW


% \begin{itemize}
% \item Underlying idea: what kind of \emph{structure} in inference
%   problems does this take advantage of? Beyond just low-rank in the
%   LIS sense. No assumption of low-dimensionality in the likelihood;
%   convergence (given condition on $t$) for even $r=1$. Relationship to
%   matching pursuit. \todo{OZ fills in here!}
% \item Generality of the method; how it can be used. We use lazy triangular
%   maps here, but could do many other things instead.
% \end{itemize}

% \todo[inline]{OLD INTRO STARTS HERE}

% The solution of many sstatistical inference problems require the
% evaluation of integrals $I[f]=\int f({x}) \pi(\d{x})$
% with respect to some \textit{intractable} distribution $\pi$\footnote{
%   In the following we will consider only distributions $\pi$ that have a
%   Radon–Nikodym derivative with respect to the Lebesgue measure, and
%   will use the notation $\pi$ to refer to both the distribution and
%   the associated density.
% }.
% The intractability of the distribution $\pi$ is to be intended as 
% the inability to generate a sample
% $\{{x}_i\}_{i=1}^n \iidsim \pi$
% with a computational time that is proportional to the generation of an
% i.i.d. sample from $\mathcal{N}(0,{\bf I}_d)$.
% In turn, this renders the Monte-Carlo approximation
% $I[f]\approx \mathcal{Q}_n[f] := n^{-1} \sum_{i=1}^{n}f({x}_i)$
% challenging.

% These distributions often occur in problems of inference of a
% parameter $x$, where
% the non-trivial assimilation of evidence $y$ can result in a complex
% update of the prior belief $\pi(x)$ through the Bayes rule
% \begin{equation}\label{eq:PosteriorDensity}
%  \pi(x\vert y) \propto \mathcal{L}_y(x) \pi(x),
% \end{equation}
% where $\mathcal{L}(x)$ is the likelihood function, that is the
% probability density function of $y$ conditioned on $x$.
% Likelihood functions are often known up to a multiplicative constant,
% which further complicates the task of generating samples from $\pi$.

% We tackle this problem by the identification of a
% diffeomorphism\footnote{
%   In general $T$ does not need to be a diffeomorphism, but only a
%   particular invertible map; see Appendix \ref{app:triangular-maps}
%   for more details. The distributions we will consider in this paper, however, fulfill the necessary
%   conditions for $T$ to be differentiable almost everywhere.
% }
% $T:\mathbb{R}^d\rightarrow\mathbb{R}^d$ characterizing the coupling
% $(\rho,\pi)$ between a \textit{tractable} distribution $\rho$ 
% and the intractable distribution $\pi$,
% meaning that $T$ is such that $\rho(A)=\pi(T(A))$ for any measurable set $A$.
% We will say that the transport $T$ \textit{pushes-forward}
% the distribution $\rho$ to the distribution $\pi$,
% and we will write $T_\sharp\rho=\pi$.
% By an abuse of notation the density associated to $\pi$ is has the
% form $T_\sharp\rho := \rho \circ T^{-1}(x) \vert \nabla T^{-1}(x)
% \vert$.
% We will equivalently say that $T$ \textit{pulls-back} the
% distribution $\pi$ to the distribution $\rho$ and write
% $T^\sharp\pi(x) := (T^{-1})_\sharp\pi(x)$.

% The availability of the transport $T$ renders the integration with respect to
% $\pi$ tractable, in fact it defines the change of variables
% $I[f]=\int f({x}) \pi(\d{x}) = \int f \circ T({x}) \rho(\d{x})$,
% which results in an integral with respect to the tractable distribution
% $\rho$.
% The distribution $\rho$ is a degree of freedom of the problem, and
% its choice, as we will see in the following,
% is driven by computational and practical requirements.

% In general there exist many maps such that $T_\sharp\rho=\pi$, but for
% practical reasons only maps with specific structures are
% computationally tractable: a non exhaustive list includes triangular
% transport maps
% \cite{el2012bayesian,spantini2018inference,bigoni2016nips},
% normalizing flows \cite{tabak2013family,rezende2015variational},
% Stein flows \cite{liu2016stein,Detommaso2018,Chen2019},
% autoregressive flows \cite{Kingma2016},
% neural ordinary differential equations \cite{Chen2018,Dupont2019}
% \todo{DB: add some literature (normalizing flow)}.
% The choice of a particular class of transports depends from its
% approximation power as well as the cost selected to identify the
% one such that $T_\sharp\rho\approx\pi$.

% In this work we will seek $T$ in a
% class of low-dimensional transport maps whose action is confined to
% carefully selected subspaces of the parameter space.
% For some prescribed tolerance $\varepsilon>0$,
% our goal is to find a map $T$ in this approximation class,
% such that the Kullback-Leibler (KL) divergence satisfies
% \begin{equation}\label{eq:KLDivergence}
%   \Dkl( \pi || T_{\sharp}\rho ) =
%   \int\log\left( \frac{\pi(x)}{T_{\sharp}\rho(x)}\right) \pi(x) \d x \leq \varepsilon \;.
% \end{equation}

% In Section \ref{sec:LazyMaps} we show how to build such a map in a set of computationally feasible map that we call lazy maps. However, the complexity to reach \eqref{eq:KLDivergence} might be large if $\varepsilon$ is too small. In this case, we show in Section \ref{sec:LayersLazyMaps} how to reach \eqref{eq:KLDivergence} via the composition of many lazy maps.


% Because of the greedy/sequential approach, we don't need to put lots of effort into approximating $H$. 




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> arXiv v2/intro_wed530.tex <==
\section{Introduction}

% Inference in the Bayesian setting typically requires the computation of integrals $\int f({x}) \pi({x}) \d{x}$, where $\pi$
% %
% is the density\footnote{In this paper, we only consider distributions that are absolutely
%   continuous with respect to the Lebesgue measure on $\mathbb{R}^d$, and thus
%   will use the notation $\pi$ to denote both the distribution and
%   its associated density.}  
% of some analytically \textit{intractable} (posterior) distribution which is known up to a normalizing constant.
Inference in the Bayesian setting typically requires the computation of integrals $\int f  \, \d\pi$  over an \textit{intractable} posterior distribution whose density\footnote{In this paper, we only consider distributions that are absolutely continuous with respect to the Lebesgue measure on $\mathbb{R}^d$, and thus will use the notation $\pi$ to denote both the distribution and its associated density.} $\pi$ is known up to a normalizing constant.
%
One approach to this problem is to construct a
deterministic nonlinear transformation, i.e., a \emph{transport map}
\cite{villani2008optimal}, \todo{took out the NF mention here since we describe it immediately below}
%, also referred to as a normalizing flow (see \cite{papamakarios2019normalizing,otherNFreview} for an overview), 
that induces a coupling of $\pi$ with a tractable distribution
$\rho$ (e.g., a standard Gaussian).
Formally, we seek a map $T$ that pushes forward $\rho$ to $\pi$, written as $T_\sharp \rho = \pi$, such that the change of variables
$\int f \, \d \pi = \int f \circ T \, \d \rho $ makes integration
tractable.

Many constructions for such maps have been developed in recent years. Normalizing flows (see \cite{rezende2015variational,tabak2013family,papamakarios2019normalizing,kobyzev2020normalizing} and references therein) build transport maps via a deep composition of functions parameterized by neural networks, 
with certain ansatzes 
% while enforcing certain structure
 to enable efficient computation. Many recently proposed autoregressive flows (for example \cite{Kingma2016,jaini2019sum}) compose triangular maps, which allow for efficient evaluation of the Jacobian determinants. In general, triangular maps \cite{bogachev2005triangular,rosenblatt1952remarks,knothe1957contributions} are
sufficiently general to couple any absolutely continuous pair of
distributions $(\rho, \pi)$, and their numerical approximations have
been investigated in \cite{el2012bayesian,marzouk2016introduction, spantini2018inference, Jaini2019}. The flow map of a neural ordinary differential equation \cite{Chen2018,Dupont2019,gholaminejad2019anode} can also been seen as an infinite-layer limit of a normalizing flow.
% that can reduce the complexity of density estimation. 
Alternatively, Stein variational methods \cite{liu2016stein,liu2017stein,Detommaso2018} provide a nonparametric way of constructing $T$ as a composition of functions lying in a chosen RKHS.
%
Many of these constructions are useful not only for variational inference 
%(e.g., approximating $\pi$ by $T_\sharp \rho$ in the sense of Kullback--Leibler (KL) divergence) 
but also for density estimation 
%(i.e., approximating $\pi$ by $\widehat{S}^{-1}_\sharp \rho$ where the map  $\widehat{S} = \widehat{T}^{-1}$  is estimated given a sample from $\pi$)
 \cite{laparra2011iterative,tabak2010density,dinh2016density}. \todo{We could remove this last sentence if tight on space, and scatter the citations around as needed.}

In general, it can be difficult to represent expressive maps in high dimensions. For example, triangular maps on $\mathbb{R}^d$ must describe $d$-variate functions and thus immediately encounter the curse of dimensionality. Similarly, kernel-based methods lose expressiveness in high dimensions \cite{Detommaso2018,Chen2019}. Flow-based methods often increase expressiveness by adding layers, but this is typically performed in an ad hoc or unstructured way, which also requires tuning. \todo{I wanted to convey the idea that layers are added rather generically, in an unfocused way, and that tuning shows up in multiple places.}

Here we propose a framework for inference that creates target-informed architectures around \emph{any} class of transport maps or normalizing flows. In particular, our framework uses rigorous \textit{a priori} error bounds to discover and exploit low-dimensional structure in a given target distribution. It also provides a methodology for efficiently solving high-dimensional inference problems via greedily constructed compositions of \emph{structured} low-dimensional maps. \todo{I think this paragraph is sharper. I wanted to inject the notion of architecture, and highlight the use of a rigorous a priori bound.}

The impact of our approach rests on two observations. 
%
First, the coordinate basis in which one expresses a transport map (i.e., $T(x)$ versus $U T(x)$, where $U$ is a rotation on $\R^d$) can 
% drastically change
strongly affect
% \todo{pretty strong there. OK, or should we say ``significantly affect'' ``strongly affect''}
 the training behavior and final performance of the method. Our framework identifies an ordered basis that best reveals a certain low-dimensional structure in the problem. Expressing the transport map in this basis focuses the expressiveness of the underlying transport class and allows for principled dimension reduction. This basis is identified by minimizing an upper bound on the Kullback--Leibler (KL) divergence between $\pi$ and its approximation, which follows from logarithmic Sobolev inequalities (see \cite{zahm2018certified}) relating the KL divergence to gradients of the target density. % via an {average derivative functional} \cite{samarov1993exploring}.

% mention GREEDY
Second, in the spirit of normalizing flows, we seek to increase the expressiveness of a transport map using repeated compositions. Rather than specifying the length of the flow before training, we increase the length of the flow sequentially. For each layer, we apply the framework above to a \emph{residual} distribution that captures the deviation between the target distribution and its current approximation. We prove weak convergence of this greedy approach to the target distribution under reasonable assumptions. This sequential framework enables efficient layer-wise training of high-dimensional maps, which especially helps control the curse of dimensionality in certain transport classes. As we shall demonstrate empirically, the greedy composition approach can further improve accuracy at the end of training, compared to baseline methods. 


%({\bf I think I capture this section above, except for information on where the bound comes from. I dont think that is needed here.})
% We considers maps are low-dimensional in
%that the transformation is restricted to a low-dimensional subspace of the
%parameter space; thus they are termed ``lazy.'' We identify the low-dimensional subspaces sequentially, by greedily minimizing a bound on the KL divergence between $\pi$ and its approximation. The bound itself follows from
%logarithmic Sobolev inequalites (see \cite{zahm2018certified})
%relating the KL divergence to gradients of the target density. We
%prove weak convergence of this approach to the target distribution,
%given even suboptimal choices of the subspace.
%
%


%{\bf I'm not sure if we need to this, it seems out of context in the intro (they don't know what low dimensional structure is yet) -->}
%We point out that while the lazy framework is able to identify and efficient capture exact low dimensional structure in a problem, the overall approach does not require the problem to be specifically structured. We also emphasize that our overall approach does not require any \emph{global} low dimensionality in the likelihood function (as in \cite{cui2014likelihood,Chen2019}, for example).%: rather, it can converge even for maps that act on a single direction at a time, despite $\pi$ and $\rho$ differing in all directions.

% despite the difference between $\pi$ and $\rho$ not being confined to a low-dimensional subspace. 


% \section{Preliminaries}

\paragraph{Preliminaries.} We will consider target distributions with densities $\pi$ on $\mathbb{R}^d$ that are differentiable almost everywhere and that can be evaluated up to a normalizing constant. Such a target will often be the posterior of a Bayesian inference problem, e.g.,
\begin{equation}\label{eq:PosteriorDensity}
 \pi(x) \coloneqq p(x\vert y) \propto \mathcal{L}_y(x) \pi_0(x),
\end{equation}
where $\mathcal{L}_y(x) \coloneqq p(y \vert x)$ is the likelihood function and $\pi_0$ is the prior. We denote the standard Gaussian density on $\mathbb{R}^d$ as $\rho$. We will consider maps $T: \mathbb{R}^d \to \mathbb{R}^d$ that are diffeomorphisms,\footnote{In general $T$ does not need to be a diffeomorphism, but only a
  particular invertible map; see Appendix \ref{app:triangular-maps}
  for more details. The distributions we will consider in this paper, however, fulfill the necessary
  conditions for $T$ to be differentiable almost everywhere.}
and with some abuse of notation, we will write the pushforward density of $\rho$ under $T$ as $T_\sharp\rho(x) \coloneqq \rho \circ T^{-1}(x) \vert \nabla T^{-1}(x) \vert$. We will frequently also use the notion of a \emph{pullback} distribution or density, written as $T^\sharp\pi \coloneqq (T^{-1})_\sharp\pi$.

%{\bf Before:}
%Our goal is to find a map $T$ that satisfies  $\Dkl( \pi || T_{\sharp}\rho ) \leq \varepsilon$ for some prescribed tolerance $\varepsilon > 0$. In Section \ref{sec:LazyMaps} we show how to build a single map in the ``lazy'' format described above. However, the map complexity needed to satisfy the prescribed tolerance might be large if $\varepsilon$ is too small. We thus show in Section \ref{sec:LayersLazyMaps} how to improve our approximations by greedily composing many lazy maps.

In \S\ref{sec:LazyMaps} we show how to build a single map in the low-dimensional ``lazy'' format described above, and describe the class of posterior distributions that admit such structure. In \S\ref{sec:LayersLazyMaps} we develop a greedy algorithm for building deep compositions of lazy maps, which effectively decomposes any inference problem into a series of lower-dimensional problems. 
% Each layer of such a map is constructed to transform the base distribution along a subspace we learn to be most important to improving the performance of the map. 
\S\ref{sec:NumericalExamples} presents numerical experiments highlighting the benefits of the lazy framework.
%
While our numerical experiments employ inverse autoregressive flows \cite{IAF} and polynomial transport maps \cite{SoS,us} as the underlying transport classes, we emphasize that the lazy framework is applicable to any class of transport. The complexity of the map, and hence the computational effort, can be tailored at each layer, making the method exceptionally flexible. \todo{Possibly omit one or two last sentences.}


%% REVISED STUFF ABOVE
% %% OLD STUFF (source material) BELOW


% \begin{itemize}
% \item Underlying idea: what kind of \emph{structure} in inference
%   problems does this take advantage of? Beyond just low-rank in the
%   LIS sense. No assumption of low-dimensionality in the likelihood;
%   convergence (given condition on $t$) for even $r=1$. Relationship to
%   matching pursuit. \todo{OZ fills in here!}
% \item Generality of the method; how it can be used. We use lazy triangular
%   maps here, but could do many other things instead.
% \end{itemize}

% \todo[inline]{OLD INTRO STARTS HERE}

% The solution of many sstatistical inference problems require the
% evaluation of integrals $I[f]=\int f({x}) \pi(\d{x})$
% with respect to some \textit{intractable} distribution $\pi$\footnote{
%   In the following we will consider only distributions $\pi$ that have a
%   Radon–Nikodym derivative with respect to the Lebesgue measure, and
%   will use the notation $\pi$ to refer to both the distribution and
%   the associated density.
% }.
% The intractability of the distribution $\pi$ is to be intended as 
% the inability to generate a sample
% $\{{x}_i\}_{i=1}^n \iidsim \pi$
% with a computational time that is proportional to the generation of an
% i.i.d. sample from $\mathcal{N}(0,{\bf I}_d)$.
% In turn, this renders the Monte-Carlo approximation
% $I[f]\approx \mathcal{Q}_n[f] := n^{-1} \sum_{i=1}^{n}f({x}_i)$
% challenging.

% These distributions often occur in problems of inference of a
% parameter $x$, where
% the non-trivial assimilation of evidence $y$ can result in a complex
% update of the prior belief $\pi(x)$ through the Bayes rule
% \begin{equation}\label{eq:PosteriorDensity}
%  \pi(x\vert y) \propto \mathcal{L}_y(x) \pi(x),
% \end{equation}
% where $\mathcal{L}(x)$ is the likelihood function, that is the
% probability density function of $y$ conditioned on $x$.
% Likelihood functions are often known up to a multiplicative constant,
% which further complicates the task of generating samples from $\pi$.

% We tackle this problem by the identification of a
% diffeomorphism\footnote{
%   In general $T$ does not need to be a diffeomorphism, but only a
%   particular invertible map; see Appendix \ref{app:triangular-maps}
%   for more details. The distributions we will consider in this paper, however, fulfill the necessary
%   conditions for $T$ to be differentiable almost everywhere.
% }
% $T:\mathbb{R}^d\rightarrow\mathbb{R}^d$ characterizing the coupling
% $(\rho,\pi)$ between a \textit{tractable} distribution $\rho$ 
% and the intractable distribution $\pi$,
% meaning that $T$ is such that $\rho(A)=\pi(T(A))$ for any measurable set $A$.
% We will say that the transport $T$ \textit{pushes-forward}
% the distribution $\rho$ to the distribution $\pi$,
% and we will write $T_\sharp\rho=\pi$.
% By an abuse of notation the density associated to $\pi$ is has the
% form $T_\sharp\rho := \rho \circ T^{-1}(x) \vert \nabla T^{-1}(x)
% \vert$.
% We will equivalently say that $T$ \textit{pulls-back} the
% distribution $\pi$ to the distribution $\rho$ and write
% $T^\sharp\pi(x) := (T^{-1})_\sharp\pi(x)$.

% The availability of the transport $T$ renders the integration with respect to
% $\pi$ tractable, in fact it defines the change of variables
% $I[f]=\int f({x}) \pi(\d{x}) = \int f \circ T({x}) \rho(\d{x})$,
% which results in an integral with respect to the tractable distribution
% $\rho$.
% The distribution $\rho$ is a degree of freedom of the problem, and
% its choice, as we will see in the following,
% is driven by computational and practical requirements.

% In general there exist many maps such that $T_\sharp\rho=\pi$, but for
% practical reasons only maps with specific structures are
% computationally tractable: a non exhaustive list includes triangular
% transport maps
% \cite{el2012bayesian,spantini2018inference,bigoni2016nips},
% normalizing flows \cite{tabak2013family,rezende2015variational},
% Stein flows \cite{liu2016stein,Detommaso2018,Chen2019},
% autoregressive flows \cite{Kingma2016},
% neural ordinary differential equations \cite{Chen2018,Dupont2019}
% \todo{DB: add some literature (normalizing flow)}.
% The choice of a particular class of transports depends from its
% approximation power as well as the cost selected to identify the
% one such that $T_\sharp\rho\approx\pi$.

% In this work we will seek $T$ in a
% class of low-dimensional transport maps whose action is confined to
% carefully selected subspaces of the parameter space.
% For some prescribed tolerance $\varepsilon>0$,
% our goal is to find a map $T$ in this approximation class,
% such that the Kullback-Leibler (KL) divergence satisfies
% \begin{equation}\label{eq:KLDivergence}
%   \Dkl( \pi || T_{\sharp}\rho ) =
%   \int\log\left( \frac{\pi(x)}{T_{\sharp}\rho(x)}\right) \pi(x) \d x \leq \varepsilon \;.
% \end{equation}

% In Section \ref{sec:LazyMaps} we show how to build such a map in a set of computationally feasible map that we call lazy maps. However, the complexity to reach \eqref{eq:KLDivergence} might be large if $\varepsilon$ is too small. In this case, we show in Section \ref{sec:LayersLazyMaps} how to reach \eqref{eq:KLDivergence} via the composition of many lazy maps.


% Because of the greedy/sequential approach, we don't need to put lots of effort into approximating $H$. 




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> arXiv v2/layers-lazy-maps.tex <==
\section{Deeply lazy maps}\label{sec:LayersLazyMaps}


\begin{algorithm}[t]
  \caption{
    Construction of a deeply lazy map
  }
  \begin{algorithmic}[1]
    \Procedure{LayersOfLazyMaps}{$\pi$, $\rho$, $\varepsilon$, $r$, $\ell_{{\text{max}}}$}
    \State Set $\pi_0=\pi$ and $\ell=0$
    \While{$\ell \leq \ell_{{\text{max}}}$ and $\frac{1}{2}\trace(H_{\ell})\geq \varepsilon$}
        \State $\ell\gets\ell+1$
        \State Compute $T_\ell  = $ \textsc{LazyMap}($\pi_{\ell-1}$, $\rho$, $0$, $r$) \Comment{Algorithm \ref{alg:LazyMap}} 
        \State Update $\frak{T}_{\ell}=\frak{T}_{\ell-1}\circ T_\ell$ 
        \State Compute $\pi_\ell = (\frak{T}_{\ell})^\sharp \pi$ 
        \State Compute $H_{\ell}=\int (\nabla\log\frac{\pi_\ell}{\rho} )(\nabla\log\frac{\pi_\ell}{\rho} )^\top\d\pi_\ell$
    \EndWhile
    
    \State\Return $\frak{T}_\ell=T_1\circ\cdots\circ T_\ell$
    \EndProcedure
  \end{algorithmic}\label{alg:LayersOfLazyMaps}
\end{algorithm}



The restriction $r\leq r_{{\text{max}}}$ in Algorithm \ref{alg:LazyMap} helps control the computational cost of constructing the lazy map, but unless a problem admits sufficient lazy structure, $T_\sharp\rho$ may not adequately approximate the posterior. To extend the numerical benefits of the lazy framework to general problems, we consider the ``deeply lazy'' map $\frak{T}_\ell$, a composition of $\ell$ lazy maps:
\[
 \frak{T}_\ell = T_1\circ\hdots\circ T_\ell ,
 \quad T_k \in\mathcal{T}_{r}(U^{k}) ,
\]
where each $T_k$ is a lazy map associated with a different unitary matrix $U^k\in\R^{d\times d}$.
For simplicity we consider the case where each lazy layer $T_k$ has the same rank $r$,
%$r = r_{{\text{max}}}$, 
though it is trivial to allow the ranks to vary from layer to layer.
%
In general, the composition of lazy maps is not itself a lazy map. For example, there exists $U^1\neq U^2$ such that $\frak{T}_2=T_1\circ T_2$ can depend nonlinearly on each input variable and so $\frak{T}_2$ cannot be written as in \eqref{eq:LazyMap}. 

% Also, approximations of the form of $(\frak{T}_\ell)_\sharp\rho$ are different than those constructed by projection pursuit \cite{huber1985projection}. \todo{flag to remove the second sentence and join the first with the preceding par}

% We note that are different than those constructed by projection pursuit \cite{huber1985projection}
%Notice also that there is no chance in general to write $(\frak{T}_\ell)_\sharp\rho(x)$ as a product $f_1( U^{1\top}_{r} x) \cdots f_\ell( U^{\ell \top}_{r} x)\rho(x)$; otherwise, by Proposition \ref{prop:CaracterizationOfLazyMaps}, $\frak{T}_\ell$ would be a lazy map with rank bounded by $r \ell$. As a consequence, approximations of the form of $(\frak{T}_\ell)_\sharp\rho$ are different than those constructed by projection pursuit \cite{huber1985projection}.

The diagnostic matrix $H$ allows us to build deeply lazy maps in a greedy way.
After $\ell-1$ iterations, the composition of maps
$\frak{T}_{\ell-1}=T_1\circ\hdots\circ T_{\ell-1}$ has been
constructed.
We seek a unitary matrix $U^{\ell}\in\R^{d\times d}$ and a lazy map $T_{\ell}\in\mathcal{T}_r(U^{\ell})$ such that $(\frak{T}_{\ell-1} \circ  T_\ell)_\sharp\rho$ best improves over  $(\frak{T}_{\ell-1})_\sharp\rho$ as an approximation to the posterior. To this end, we define the residual distribution
\[ 
\pi_{\ell-1} = (\frak{T}_{\ell-1})^\sharp \pi,
\]
i.e., the pullback of $\pi$ through the current transport map $\frak{T}_{\ell-1}$.
Note that $\Dkl( \pi||(\frak{T}_{\ell-1} \circ  T_\ell)_\sharp \rho) = \Dkl( \pi_{\ell-1} ||(T_\ell)_\sharp \rho)$. We thus build $T_\ell$ using Algorithm \ref{alg:LazyMap}, replacing the posterior $\pi$ by the residual distribution $\pi_{\ell-1}$.
We then update the transport map to be $\frak{T}_{\ell}=\frak{T}_{\ell-1}\circ T_\ell$ and the residual density $\pi_\ell = (\frak{T}_{\ell})^\sharp \pi$. 


We note that applying Proposition \ref{prop:LogSobResult} to $\pi_\ell$ with $r=0$ yields
 \[
 \Dkl(\pi||(\frak{T}_\ell)_\sharp\rho)=\Dkl(\pi_\ell||\rho)\leq \frac{1}{2}(\lambda_1+\cdots+\lambda_d)=\frac{1}{2}\trace(H_{\ell}),
 \]
 where we define the diagnostic matrix at iteration $\ell$ as, 
% \todo{Just a note, first def of H is inline. Maybe we switch so first def in out of line and this is inline}
\[ 
H_{\ell}=\int \left (\nabla\log\frac{\pi_\ell}{\rho} \right ) \left (\nabla\log\frac{\pi_\ell}{\rho}  \right )^\top\d\pi_\ell.
\]
% We see that $\frac12 \trace{(H_\ell)}$ provides an independently useful error bound on the forward KL divergence, applicable to \emph{any} flow-based method.
% Our framework naturally exposes the error bound  $\frac12 \trace{(H_\ell)}$, which can be used to evaluate performance in terms of the forward KL divergence, applicable to \emph{any} flow-based method.
Our framework thus naturally exposes the error bound  $\frac12 \trace{(H_\ell)}$ on the forward KL divergence, which is of {independent} interest and applicable to \emph{any} flow-based method. We refer to this bound as the \emph{trace diagnostic}.

%
This bound can also be used as a stopping criterion for the greedy algorithm; one can continue adding layers until the bound falls below some desired threshold. 
%
This construction is summarized in Algorithm \ref{alg:LayersOfLazyMaps}, and details on its numerical implementation are given in Appendix~\ref{app:numerical-algorithms}.

%  (As written, this algorithm would compute the matrix $H_\ell$ twice: once in step 8
% and once in step 2 of Algorithm \ref{alg:LazyMap} at the next
% iteration. Of course, the actual implementation of this algorithm
% reuses this information.)\todo{db: we may find a
%   way to remove the last two sentences and maybe refer to the actual
%   implementation in the appendix?}



The next proposition gives a sufficient condition on $U^\ell$ to guarantee the convergence of our greedy algorithm. The proof is given in Appendix \ref{proof:GreedyConvergence_condition}.
\begin{proposition}\label{prop:GreedyConvergence_condition}
 Let $U^1,U^2,\hdots$ be a sequence of unitary matrices.
 For any $\ell\geq1$, we let $T_\ell \in\mathcal{T}_r(U^\ell)$ be a lazy map that minimizes $\Dkl( \pi_{\ell-1} ||(T_\ell)_\sharp \rho)$, where $\pi_{\ell-1} = (T_1\circ\hdots\circ T_{\ell-1})^\sharp \pi$.
 If there exists $0< t\leq 1$ such that for any $\ell\geq1$
 \begin{equation}\label{eq:GreedyConvergence_condition}
  \Dkl( (U_r^{\ell \top})_\sharp \pi_{\ell-1} || \rho_r )
  \,\geq\, t  \sup_{\substack{ U\in\R^{d\times d} \\ \text{s.t.} \ UU^\top=I_d}} \Dkl( (U_r^\top)_\sharp \pi_{\ell-1} || \rho_r ),
 \end{equation}
 
 then $(T_1\circ\hdots\circ T_\ell)_\sharp\rho $ converges weakly to $\pi$.
\end{proposition}
%\todo{Reviewer addition: Add point that the condition must apply simultaneously to all layers}
Let us comment on the condition \eqref{eq:GreedyConvergence_condition}. Recall that the unitary matrix $U$ that maximizes $\Dkl( (U_r^\top)_\sharp \pi_{\ell-1} || \rho_r )$ is optimal; see \eqref{eq:KL_Tstar_Decomp}.
 % with $\pi$ replaced by $\pi_{\ell-1}$
By \eqref{eq:GreedyConvergence_condition}, the case $t=1$ means that $U^\ell$ is optimal at each iteration. This corresponds to an
\textit{ideal} greedy algorithm. The case $0<t<1$ allows suboptimal
choices for $U^\ell$ without losing the convergence property of the
algorithm. Such a greedy algorithm converges even with a
potentially crude selection of $U^\ell$ that corresponds to a $t$
close to zero. This also is why an approximation to
$H_\ell$ is expected to be sufficient; see Section
\ref{sec:NumericalExamples}. 
%
We emphasize that condition \eqref{eq:GreedyConvergence_condition} must apply simultaneously to \emph{all} layers for a given $0<t\leq1$. Following \cite{Temlyakov2011}, one could relax this condition
% condition \eqref{eq:GreedyConvergence_condition} 
by replacing $t$ with a sequence $(t_\ell)$ that goes to zero sufficiently slowly. This development is left for future work.
% \todo{we write this concept twice, also in the previous section. YM: that's okay!}
%
% \todo{Note on $t_\ell$ may not be in scope here. This is saying we could be more or less optimal at each lazy layer, and still converge correct?}Following \cite{Temlyakov2011}, one can further relax the
% condition \eqref{eq:GreedyConvergence_condition} by replacing $t$ with a
% non-constant parameter $t_\ell$ which can go to zero under certain conditions. This development is left for future work.
%
Finally, note that Proposition \ref{prop:GreedyConvergence_condition} does not require any constraints on $r$, so we have convergence even with $r=1$, where each layer only acts on a single direction at a time. %Of course, larger $r$ yields faster convergence





%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> arXiv v2/layers-lazy-mapsCONF.tex <==
\section{Layers of lazy maps}\label{sec:LayersLazyMaps}


\begin{algorithm}[t]
  \caption{
    Compute layers of lazy maps
  }
  \begin{algorithmic}[1]
    \Procedure{LayersOfLazyMaps}{$\pi$, $\rho$, $\varepsilon$, $r$, $\ell_{{\text{max}}}$}
    \State Set $\pi_0=\pi$ and $\ell=0$
    \While{$\ell \leq \ell_{{\text{max}}}$ and $\frac{1}{2}\trace(H_{\ell})\geq \varepsilon$}
        \State $\ell\gets\ell+1$
        \State Compute $T_\ell  = $ \textsc{LazyMap}($\pi_{\ell-1}$, $\rho$, $0$, $r$) \Comment{Algorithm \ref{alg:LazyMap}} 
        \State Update $\frak{T}_{\ell}=\frak{T}_{\ell-1}\circ T_\ell$ 
        \State Compute $\pi_\ell = (\frak{T}_{\ell})^\sharp \pi$ 
        \State Compute $H_{\ell}=\int (\nabla\log\frac{\pi_\ell}{\rho} )(\nabla\log\frac{\pi_\ell}{\rho} )^\top\d\pi_\ell$
    \EndWhile
    
    \State\Return $\frak{T}_\ell=T_1\circ\cdots\circ T_\ell$
    \EndProcedure
  \end{algorithmic}\label{alg:LayersOfLazyMaps}
\end{algorithm}



The restriction $r\leq r_{{\text{max}}}$ in Algorithm \ref{alg:LazyMap} helps control the computational cost of constructing the lazy map, but unless a problem admits sufficient lazy structure, $T_\sharp\rho$ may not adequately approximate the posterior. To extend the numerical benefits of the lazy framework to general problems, we consider the ``deeply lazy'' map $\frak{T}_\ell$, a composition of $\ell$ lazy maps:
\[
 \frak{T}_\ell = T_1\circ\hdots\circ T_\ell ,
 \quad T_k \in\mathcal{T}_{r}(U^{k}) ,
\]
where each $T_k$ is a lazy map associated with a different unitary matrix $U^k\in\R^{d\times d}$.
For simplicity we consider the case where each lazy layer $T_k$ has the same rank $r$,
%$r = r_{{\text{max}}}$, 
though it is trivial to allow the ranks to vary from layer to layer.

In general, the composition of lazy maps is not itself a lazy map. For example, there exists $U^1\neq U^2$ such that $\frak{T}_2=T_1\circ T_2$ might depend nonlinearly on each input variable and so it cannot be written as in \eqref{eq:LazyMap}. Also, approximations of the form of $(\frak{T}_\ell)_\sharp\rho$ are different than those constructed by projection pursuit \cite{huber1985projection}.\todo{Maybe we have have an explanation in an appendix} %
% We note that are different than those constructed by projection pursuit \cite{huber1985projection}
%Notice also that there is no chance in general to write $(\frak{T}_\ell)_\sharp\rho(x)$ as a product $f_1( U^{1\top}_{r} x) \cdots f_\ell( U^{\ell \top}_{r} x)\rho(x)$; otherwise, by Proposition \ref{prop:CaracterizationOfLazyMaps}, $\frak{T}_\ell$ would be a lazy map with rank bounded by $r \ell$. As a consequence, approximations of the form of $(\frak{T}_\ell)_\sharp\rho$ are different than those constructed by projection pursuit \cite{huber1985projection}.

The diagnostic matrix $H$ allows us to build deeply lazy maps in a greedy way.
After $\ell-1$ iterations, the composition of maps
$\frak{T}_{\ell-1}=T_1\circ\hdots\circ T_{\ell-1}$ has been
constructed.
We seek a unitary matrix $U^{\ell}\in\R^{d\times d}$ and a lazy map $T_{\ell}\in\mathcal{T}_r(U^{\ell})$ such that $(\frak{T}_{\ell-1} \circ  T_\ell)_\sharp\rho$ best improves over  $(\frak{T}_{\ell-1})_\sharp\rho$ as an approximation to the posterior. To this end, we define the residual distribution
\[ 
\pi_{\ell-1} = (\frak{T}_{\ell-1})^\sharp \pi,
\]
i.e., the pullback of $\pi$ through the current transport map $\frak{T}_{\ell-1}$.
Note that $\Dkl( \pi||(\frak{T}_{\ell-1} \circ  T_\ell)_\sharp \rho) = \Dkl( \pi_{\ell-1} ||(T_\ell)_\sharp \rho)$. We thus build $T_\ell$ using Algorithm \ref{alg:LazyMap}, replacing the posterior $\pi$ by the residual distribution $\pi_{\ell-1}$.
We then update the transport map to be $\frak{T}_{\ell}=\frak{T}_{\ell-1}\circ T_\ell$ and the residual density $\pi_\ell = (\frak{T}_{\ell})^\sharp \pi$. 


We note that applying Proposition \ref{prop:LogSobResult} to $\pi_\ell$ with $r=0$ yields
 \[
 \Dkl(\pi||(\frak{T}_\ell)_\sharp\rho)=\Dkl(\pi_\ell||\rho)\leq \frac{1}{2}(\lambda_1+\cdots+\lambda_d)=\frac{1}{2}\trace(H_{\ell}),
 \]
 where we define the diagnostic matrix at iteration $\ell$ as, 
\[ 
H_{\ell}=\int \left (\nabla\log\frac{\pi_\ell}{\rho} \right ) \left (\nabla\log\frac{\pi_\ell}{\rho}  \right )^\top\d\pi_\ell.
\]
%
We see that $\frac12 \trace{(H_\ell)}$ provides an independently useful error bound \todo{Sharpen further? Want to highlight that this is a new and very broadly applicable bound, of independent interest!} on the forward KL divergence, applicable to \emph{any} flow-based method. Here it can be used as a stopping criterion for the greedy algorithm: continue adding layers until the bound falls below some desired threshold. 
%
This construction is summarized in Algorithm \ref{alg:LayersOfLazyMaps}, and details on its numerical implementation are given in Appendix~\ref{app:numerical-algorithms}.

%  (As written, this algorithm would compute the matrix $H_\ell$ twice: once in step 8
% and once in step 2 of Algorithm \ref{alg:LazyMap} at the next
% iteration. Of course, the actual implementation of this algorithm
% reuses this information.)\todo{db: we may find a
%   way to remove the last two sentences and maybe refer to the actual
%   implementation in the appendix?}



The next proposition gives a sufficient condition on $U^\ell$ to guarantee the convergence of our greedy algorithm. The proof is given in Appendix \ref{proof:GreedyConvergence_condition}.
\begin{proposition}\label{prop:GreedyConvergence_condition}
 Let $U^1,U^2,\hdots$ be a sequence of unitary matrices.
 For any $\ell\geq1$, we let $T_\ell \in\mathcal{T}_r(U^\ell)$ be a lazy map that minimizes $\Dkl( \pi_{\ell-1} ||(T_\ell)_\sharp \rho)$, where $\pi_{\ell-1} = (T_1\circ\hdots\circ T_{\ell-1})^\sharp \pi$.
 If there exists $0< t\leq 1$ such that for any $\ell\geq1$
 \begin{equation}\label{eq:GreedyConvergence_condition}
  \Dkl( (U_r^{\ell \top})_\sharp \pi_{\ell-1} || \rho_r )
  \,\geq\, t  \sup_{\substack{ U\in\R^{d\times d} \\ \text{s.t.} UU^\top=I_d}} \Dkl( (U_r^\top)_\sharp \pi_{\ell-1} || \rho_r ),
 \end{equation}
 
 then $(T_1\circ\hdots\circ T_\ell)_\sharp\rho $ converges weakly to $\pi$.
\end{proposition}

Let us comment on the condition \eqref{eq:GreedyConvergence_condition}. Recall that the unitary matrix $U$ that maximizes $\Dkl( (U_r^\top)_\sharp \pi_{\ell-1} || \rho_r )$ is optimal; see \eqref{eq:KL_Tstar_Decomp}.
 % with $\pi$ replaced by $\pi_{\ell-1}$
By \eqref{eq:GreedyConvergence_condition}, the case $t=1$ means that $U^\ell$ is optimal at each iteration. This corresponds to an
\textit{ideal} greedy algorithm. The case $0<t<1$ allows suboptimal
choices for $U^\ell$ without losing the convergence property of the
algorithm. Such a \textit{weak} greedy algorithm converges even with a
potentially crude selection of $U^\ell$ that corresponds to a $t$
close to zero. This also is why an approximation to
$H_\ell$ is expected to be sufficient; see Section
\ref{sec:NumericalExamples}.
% \todo{we write this concept twice, also in the previous section. YM: that's okay!}
Following \cite{Temlyakov2011}, one can further relax the
condition \eqref{eq:GreedyConvergence_condition} by replacing $t$ with a
non-constant parameter $t_\ell$ which can go to zero under certain conditions. This development is left for future work.
Finally let us note that Proposition \ref{prop:GreedyConvergence_condition} does not require any constraints on $r$, so we have convergence even with $r=1$, where each layer only acts on a single direction at a time. %Of course, larger $r$ yields faster convergence





%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> arXiv v2/macroMap.tex <==
%

%
%
%
\newcommand{\Ex}{\mathbb{E}}                                                   %
\DeclareMathOperator{\cov}{Cov}
\DeclareMathOperator{\Var}{Var}
\newcommand{\eqd}{\buildrel d \over =}                                       %
\newcommand{\Gauss}{\mathcal{N}}                                      %
\newcommand{\Unif}{\mathcal{U}}                                      %
\newcommand{\eqas}{\buildrel a.s. \over =}                                  %
\newcommand{\approxeqd}{\buildrel d \over \approx}                   %
\DeclareMathOperator\supp{supp}
\DeclareMathOperator\erf{erf}
\newcommand{\push}{_\sharp}                                      %
\newcommand{\orth}{ \perp\!\!\!\perp }  %
\newcommand{\rank}{{\rm rank}}

\newcommand{\eqdis}{\, {\buildrel d \over =} \,}

\newcommand{\borelm}{\mathscr{M}}
\newcommand{\borelmp}{\borelm_+}
\newcommand{\lebm}{\boldsymbol{\lambda} } %
\newcommand{\genm}{\boldsymbol{\nu} }	  %
\newcommand{\agenm}{\hat{\boldsymbol{\nu}}}	  %
\newcommand{\agengr}{\hat{\Gcb}}	  %


\renewcommand{\d}{\mathrm{d}}
\newcommand{\ddx}{\frac{\d}{\d x}}

%
%
%
\newcommand{\re}{\mathbb{R}}
\newcommand{\ra}{\rightarrow}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\newcommand{\bspace}{\mathcal{B}(\re^D)} %
\newcommand{\vphi}{\varphi}

%
%
%
\newcommand{\Bc}{\mathcal{B}}
\newcommand{\Cc}{\mathcal{C}}
\newcommand{\Dc}{\mathcal{D}}
\newcommand{\Xc}{\mathcal{X}}
\newcommand{\Zc}{\mathcal{Z}}
\newcommand{\Kc}{\mathcal{K}}
\newcommand{\Vc}{\mathcal{V}}
\newcommand{\Fc}{\mathcal{F}}
\newcommand{\Pc}{\mathcal{P}}
\newcommand{\Qc}{\mathcal{Q}}
\newcommand{\Ec}{\mathcal{E}}
\newcommand{\Ic}{\mathcal{I}}
\newcommand{\Ac}{\mathcal{A}}
\newcommand{\Sc}{\mathcal{S}}
\newcommand{\Wc}{\mathcal{W}}
\newcommand{\Tc}{\mathcal{T}}


%
%
%
\newcommand{\Xb}{\boldsymbol{X}}
\newcommand{\xb}{\boldsymbol{x}}
\newcommand{\Yb}{\boldsymbol{Y}}
\newcommand{\yb}{\boldsymbol{y}}
\newcommand{\Pb}{\boldsymbol{P}}
\newcommand{\Zb}{\boldsymbol{Z}}
\newcommand{\zb}{\boldsymbol{z}}
\newcommand{\eb}{\boldsymbol{e}}
\newcommand{\Fb}{\boldsymbol{F}}
\newcommand{\Hb}{\boldsymbol{H}}
\newcommand{\hb}{\boldsymbol{h}}
\newcommand{\Qb}{\boldsymbol{Q}}
\newcommand{\Rb}{\boldsymbol{R}}
\newcommand{\Gammab}{\boldsymbol{\Gamma}}
\newcommand{\Ab}{\boldsymbol{A}}
\newcommand{\ab}{\boldsymbol{a}}
\newcommand{\Bb}{\boldsymbol{B}}
\newcommand{\Cb}{\boldsymbol{C}}
\newcommand{\cb}{\boldsymbol{c}}
\newcommand{\Jb}{\boldsymbol{J}}
\newcommand{\sbb}{\boldsymbol{s}}
\newcommand{\ub}{\boldsymbol{u}}
\newcommand{\vb}{\boldsymbol{v}}
\newcommand{\Vb}{\boldsymbol{V}}
\newcommand{\Lambdab}{\boldsymbol{\Lambda}}
\newcommand{\betab}{\boldsymbol{\beta}}
\newcommand{\Lb}{\boldsymbol{L}}
\newcommand{\Sigmab}{\boldsymbol{\Sigma}}
\newcommand{\mub}{\boldsymbol{\mu}}
\newcommand{\phib}{\boldsymbol{\phi}}
\newcommand{\xib}{\boldsymbol{\xi}}
\newcommand{\kappab}{\boldsymbol{\kappa}}
\newcommand{\lambdab}{\boldsymbol{\lambda} } %
\newcommand{\Ub}{\boldsymbol{U}}
\newcommand{\Eb}{\boldsymbol{E}}
%
%
%
\newcommand{\Gcb}{\boldsymbol{\mathcal{G}}}
\newcommand{\Ccb}{\boldsymbol{\mathcal{C}}}
\newcommand{\Kcb}{\boldsymbol{\mathcal{K}}}
\newcommand{\Tcb}{\boldsymbol{\mathcal{T}}}


%
%
%
\newcommand{\Pbb}{\mathbb{P}}
\newcommand{\Nbb}{\mathbb{N}}
\newcommand{\Ibb}{\mathbb{I}}

\newcommand{\Ibf}{\mathbf{I}}


%
%
%
\newcommand{\Cfrak}{\mathfrak{C}}
\newcommand{\cfrak}{\mathfrak{c}}
\newcommand{\rfrak}{\mathfrak{r}}

%
%
%
\newcommand{\mpos}{\nu_{\text{pos}}} %
\newcommand{\dpos}{\pi} %
\newcommand{\dupos}{\bar{\pi}} %

\newcommand{\mref}{\nu_{\text{ref}}} %

%
%
%
%
\newcommand{\sparse}{ \mathfrak{I} }
\newcommand{\sparsefs}{ \mathscr{T} } %

\newcommand{\neigh}{ {\rm Nb} }
\newcommand{\fillin}{\textswab{F} } 
%
\newcommand{\permset}{\mathfrak{P} } 

%
\newcommand{\vhyp}{\boldsymbol{\Theta}}
\newcommand{\vhyps}{\theta}

\newcommand{\dhyp}{p}
\newcommand{\ddata}{d} %

\newcommand{\submap}{\mathfrak{M}}

\newcommand{\lmap}{L} %
\newcommand{\rmap}{R} %
\newcommand{\decset}{\mathfrak{D}} %


%
%
%
\newcommand{\dens}{\mathscr{P}}
\newcommand{\contpd}{\mathscr{C}_+}
\newcommand{\diffpd}{\mathscr{D}_+}

%
%
%
\newcommand{\forop}{ \Fb }
\newcommand{\noised}{ \boldsymbol{\varepsilon} }
\newcommand{\noisedcov}{ \Qb }
\newcommand{\noiseo}{ \boldsymbol{\xi} }
\newcommand{\noiseocov}{ \Rb }
\newcommand{\obsop}{ \Hb }



%
%
%
\newcommand{\Aset}{ \Ac }
\newcommand{\Bset}{ \Bc }
\newcommand{\Sset}{ \Sc }
\newcommand{\Aind}{ \Aset^\perp }
\newcommand{\Aindi}{ \mathfrak{a}_i }

\newcommand{\Adep}{ \Aset_\star }

%
%
%

%
\newcommand{\rdvs}{x}               			 %
\newcommand{\tdvs}{z}               			 %
\newcommand{\tdv}{\boldsymbol{\tdvs}}                %
\newcommand{\rdv}{\boldsymbol{\rdvs}}                %
\newcommand{\tdva}{\tdv^*}                %
\newcommand{\rdva}{\rdv^*}                %
\newcommand{\tdvsa}{\tdvs^*}                %
\newcommand{\rdvsa}{\rdvs^*}                %


\newcommand{\trv}{\boldsymbol{Z}}                %
\newcommand{\rrv}{\boldsymbol{X}}                %
\newcommand{\sri}{\rdv_i}                %
\newcommand{\sti}{\tdv_i}                %

\newcommand{\pd}{n}                %

\newcommand{\data}{ {\boldsymbol{D}} }               %
\newcommand{\datai}{ \boldsymbol{d} }               %
\newcommand{\ddim}{n_\data}    %
\newcommand{\param}{\Theta}     %
\newcommand{\paramt}{\boldsymbol{\param}}    %
\newcommand{\pdim}{n_\param} %

\newcommand{\lebMeas}{\mu_{Leb}} %
\newcommand{\ntd}{\pi}            %
\newcommand{\td}{\bar{\pi}}                  %
\newcommand{\rd}{\eta}                          %
\newcommand{\tmeas}{\mu_{\rm tar}}        %
\newcommand{\rmeas}{\mu_{\rm ref}}        %

\newcommand{\emap}{T}                          %
\newcommand{\demap}{{\nabla T}}                  %
\newcommand{\imap}{{\widetilde{T}}}       %
\newcommand{\dimap}{{\nabla \widetilde{T} }} %

\newcommand{\efmap}{S}                          %
\newcommand{\defmap}{{\nabla S}}                  %
\newcommand{\ifmap}{{\widetilde{S}}}       %
\newcommand{\difmap}{{D \widetilde{S} }} %

\newcommand{\mapp}{\gamma}                %
\newcommand{\mappa}{\bar{\mapp}}        %
\newcommand{\xst}{x_*}                      
\newcommand{\zst}{z_*}                      


%
\newcommand{\Dkl}{\mathcal{D}_{\rm KL}}         %
\newcommand{\spaceMap}{\mathcal{T}}             %
\newcommand{\spaceMapa}{\mathcal{T}_h}             %

\newcommand{\spaceMapT}{\mathcal{T}_\triangle}  %

\newcommand{\tmeasNew}{\tmeas} %
\newcommand{\rmeasNew}{\rmeas}  %
\newcommand{\ntda}{\widetilde{\pi}}                  %

%
\newcommand{\constrrefae}{, \quad(\nu_{\Xc}-\rm{a.e.})  }  
\newcommand{\constrtarae}{, \quad(\ntd-\rm{a.e.})  }  
\newcommand{\pull}{^\sharp}  
%

%
\newcommand{\dimtot}{n} %
\newcommand{\rvtot}{\trv}  %
\newcommand{\dvtot}{x}     %
\newcommand{\frv}{\boldsymbol{D}}   %

\newcommand{\rdvf}{ \rdv_{\frv}}  
\newcommand{\rdvse}{ \rdv_{\srv}}  

\newcommand{\fdv}{{\boldsymbol{d}} } 
\newcommand{\fdvs}{d} 
\newcommand{\srv}{\boldsymbol{\Theta}}  %
\newcommand{\sdv}{{\boldsymbol{\theta}}}
\newcommand{\sdvs}{ \theta }  
\newcommand{\dimfrv}{n_{\fdvs}}  
\newcommand{\dimsrv}{n_{\sdvs}}
\newcommand{\jointfs}{\ntd_{\frv,\srv}}
\newcommand{\condsgf}{\ntd_{\srv\vert\frv}}
\newcommand{\margf}{\ntd_{\frv}}
\newcommand{\condsgfd}{\ntd_{\srv\vert\frv=\fdv}}
\newcommand{\rdsrv}{\rd_{\srv}}
\newcommand{\rdfrv}{\rd_{\frv}}

\newcommand{\mop}{\mathcal{M}_d}

\newcommand{\gd}{\eta}  
\newcommand{\fv}{d}  
\newcommand{\sv}{\theta}  
\newcommand{\dimfv}{n_d}  
\newcommand{\dimsv}{n_\sv}  

\newcommand{\mapcf}{\emap^{\frv}}  
\newcommand{\mapcs}{\emap^{\srv}}  

\newcommand{\wb}{\boldsymbol{w}}  
\newcommand{\dvpl}{\wb}  
\newcommand{\solsystem}{\rdv_{\fdv}^\star}  

%%%%%%%%%%%%%%%%%% LINEAR PAPER %%%%%%%%%%%%%%%%%%%%%%%
% upper case cal
\newcommand{\Hc}{{\cal H}}
\newcommand{\Jc}{{\cal J}}
\newcommand{\Lc}{{\cal L}}
\newcommand{\Mc}{{\cal M}}
\newcommand{\Nc}{{\cal N}}
\newcommand{\Rc}{{\cal R}}
\newcommand{\Uc}{{\cal U}}

% upper case hats
\newcommand{\arrP}{\stackrel{{\rm P}}{\longrightarrow}}
\newcommand{\bias}{{\rm Bias}}
\newcommand{\C}{{\mathbb{C}}}
\newcommand{\Calxo}{{C^\alpha(x_0)}}
\def\chilam{{\chi_\lambda}}
\def\chial{{\chi_\alpha}}
\newcommand{\chialp}{{\chi_n^2(\alpha)}} 
\newcommand{\ch}{{\widehat{c}}} 
\newcommand{\cl}{{c_\lambda}}
\newcommand{\cons}{{C}}
\newcommand{\frn}{{\frac{1}{n}}}
\newcommand{\fnl}{{f_{\rm N L}}}
\newcommand{\hfxo}{{h_f(x_0)}}
\newcommand{\Lp}{{L^p}}
\newcommand{\Lploc}{{L^p_{\rm loc}}}
\newcommand{\ellp}{{\ell_\phi}}
\newcommand{\mse}{{\rm MSE}}
\newcommand{\N}{{\mathbb{N}}}
\newcommand{\Nrho}{{N_\rho(x_0)}}
\newcommand{\Ntrho}{{N_{2\rho}(x_0)}}
\newcommand{\Nr}{{N_r(x_0)}}
\newcommand{\NrJ}{{N_{r_J}(x_0)}}
\newcommand{\onev}{\boldsymbol{1}}
\newcommand{\onevp}{\onev_{\perp}}
\newcommand{\Prob}{\mathbb{P}}
\newcommand{\Qjx}{{Q_j(x_0)}}
\newcommand{\QJx}{{Q_J(x_0)}}
\newcommand{\Qlam}{{Q(\lambda)}}
\def\Ral{{R_\alpha}}
\def\rh{{\widehat r}}
\def\Sn{{\cal S}_n}
\newcommand{\ShfJ}{{\widehat{S}_{f,J}}}
\newcommand{\Tup}{{T_u^p(x_0)}}
\newcommand{\ufpxo}{{u_f^p(x_0)}}
\newcommand{\vare}{\varepsilon}
\newcommand{\xbar}{{\overline{X}}}
\def\zal2{z_{\alpha/2}}
\def\zalp{z_\alpha}
\newcommand{\Z}{{\mathbb{Z}}}
\newcommand{\R}{{\mathbb{R}}}
\newcommand{\zero}{\boldsymbol{0}}

\newcommand{\Gy}{\Gamma_{\Yb}}
\newcommand{\Gyh}{\widehat{\Gamma}_{\rm y}}
\newcommand{\Gobs}{\Gamma_{\rm obs}}
\newcommand{\Gpr}{\Gamma_{\rm pr}}

\newcommand{\Gprs}{S_{\rm pr}} %% square root of the prior covariance matrix
\newcommand{\Gprst}{S_{\rm pr}^\top} 

\newcommand{\Gposhs}{\widehat{S}_{\rm pos}}
\newcommand{\Gposs}{S_{\rm pos}}
\newcommand{\Gys}{S_{\Yb}}
\newcommand{\Hhs}{S_{ \widehat{H}}}
\newcommand{\Gobss}{S_{\rm obs}}

\newcommand{\Gpos}{\Gamma_{\rm pos}}
\newcommand{\nupos}{\nu_{\rm pos}}
\newcommand{\nuposh}{\widehat{\nu}_{\rm pos}}
\newcommand{\Gposh}{\widehat{\Gamma}_{\rm pos}}
\newcommand{\mupos}{\mu_{\rm pos}(\Yb)}
\newcommand{\muposr}{\mu_{\rm pos}^{(r)}(\Yb)}
\newcommand{\muposhr}{\widehat{\mu}_{\rm pos}^{(r)}(\Yb)}

\newcommand{\muposy}{\mu_{\rm pos}(y)}
\newcommand{\muposry}{\mu_{\rm pos}^{(r)}(y)}
\newcommand{\muposhry}{\widehat{\mu}_{\rm pos}^{(r)}(y)}

\newcommand{\df}{d_{\Fc}}
\DeclareMathOperator{\dist}{dist}
\DeclareMathOperator{\trace}{Tr}
\DeclareMathOperator{\Span}{span}


%
% lower case hats
\newcommand{\mbh}{\widehat{\boldsymbol{m}}}
\newcommand{\mbhl}{\mbh_{\lambda}}
\newcommand{\phih}{\widehat{\phi}}
\newcommand{\sigmah}{\widehat{\sigma}}
\newcommand{\thetah}{\widehat{\theta}}
% upper case hats
\newcommand{\Lmh}{\widehat{L}_m}
\newcommand{\Uh}{\widehat{U}}
% lower case bold
\newcommand{\alphab}{\boldsymbol{\alpha}}
\newcommand{\bb}{\boldsymbol{b}}
\newcommand{\bbp}{\bb_*}
\newcommand{\deltab}{\boldsymbol{\delta}}
\newcommand{\epsb}{\boldsymbol{\varepsilon}}
\newcommand{\gammab}{\boldsymbol{\gamma}}
\newcommand{\gb}{\boldsymbol{g}}
\newcommand{\mb}{\boldsymbol{m}}
\newcommand{\rb}{\boldsymbol{r}}
\newcommand{\thetab}{\boldsymbol{\theta}}
\newcommand{\wbt}{\tilde{\wb}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%% LINEAR GOAL %%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Gz}{\Gamma_{\Zb}}

\newcommand{\Gzyh}{\widehat{\Gamma}_{\Zb|\Yb}}
\newcommand{\Gzyhs}{ S_{\Zb|\Yb}}
\newcommand{\Gzyt}{\widetilde{\Gamma}_{\Zb|\Yb}}
\newcommand{\Gzyts}{\widetilde{S}_{\Zb|\Yb}}
\newcommand{\Gzysub}{\widehat{\Gamma}_{\Zb|\Yb}}
\newcommand{\Gzysubs}{\widehat{S}_{\Zb|\Yb}}
\newcommand{\Gzyopt}{\widetilde{\Gamma}_{\Zb|\Yb}}
\newcommand{\Gzyopts}{\widetilde{S}_{\Zb|\Yb}}


\newcommand{\Gzy}{ \Gamma _{\Zb|\Yb}}
\newcommand{\Geta}{ \Gamma _{\eta}}
\newcommand{\Gpi}{ \Gamma _{\pi}}

\newcommand{\nuz}{\nu_{\Zb}}

\newcommand{\muzy}{\mu_{\Zb|\Yb}(\Yb)}
\newcommand{\muzyapp}{\widetilde{\mu}_{\Zb|\Yb}(\Yb)}

\newcommand{\error}{\boldsymbol{\mathcal{E}}} 
\newcommand{\errorTr}{\boldsymbol{\Delta} }

\newcommand{\gop}{\mathcal{O}} 
\newcommand{\gopd}{\gop_\dagger} 
\newcommand{\Dom}{\mathcal{D}} 
\newcommand{\Temp}{\Theta} 
\newcommand{\Tempb}{\mathbf{\Temp}} 
\newcommand{\Tempbh}{\mathbf{\Temp}_h} 
\newcommand{\Tempbhz}{\mathbf{\Temp}_{0h}} 

\newcommand{\dr}{d_{\mathcal{R}}} 
\newcommand{\spdman}{\it{Sym}^+ } 
\newcommand{\nop}{\mathscr{J}} 
%
\newcommand{\mzy}{\nu_{\Zb \vert \Yb } }
 \newcommand{\mzya}{\tilde{\nu}_{\Zb \vert \Yb } }
\newcommand{\pizy}{\pi_{\Zb \vert \Yb } }
\newcommand{\piz}{\pi_{\Zb} }
 \newcommand{\pizya}{\tilde{\pi}_{\Zb \vert \Yb } }

 \newcommand{\sbo}{\boldsymbol{s}}
\newcommand{\fb}{\boldsymbol{f}}
\newcommand{\mupr}{\mu_\text{pr}} 
\newcommand{\Zbh}{\widehat{\Zb}} 


%%%%%%%%%%%%%%% MACRO FOR LINEAR PAPER %%%%%%%%%%%%%%%%%%%
\newcommand{\lpwopt}{\widehat{w}_i}

\newcommand{\wq}{\widehat{q}}

%%%%%%%%%%%%%%% MACRO FOR FILTERING CHAPTER %%%%%%%%%%%%%%%%%%%
\newcommand{\Zf}{ \Zb^f } %forecast random variable
\newcommand{\Zfh}{ \hat{\Zb}^f } %estimato forecast random variable

\newcommand{\Zfs}{ Z^f } %scalar forecast random variable
\newcommand{\pif}{ \pi^f } %forecast density
\newcommand{\pifh}{ \hat{\pi}^f } %estimator forecast density

\newcommand{\nens}{ p } %caridnality forecast ensemble
\newcommand{\dstate}{ n } %forecast random variable

\newcommand{\bfA}{\mathbf{A}}
\newcommand{\bfB}{\mathbf{B}}
\newcommand{\bfC}{\mathbf{C}}
\newcommand{\bfD}{\mathbf{D}}
\newcommand{\bfE}{\mathbf{E}}
\newcommand{\bfF}{\mathbf{F}}
\newcommand{\bfG}{\mathbf{G}}
\newcommand{\bfH}{\mathbf{H}}
\newcommand{\bfI}{\mathbf{I}}
\newcommand{\bfJ}{\mathbf{J}}
\newcommand{\bfK}{\mathbf{K}}
\newcommand{\bfL}{\mathbf{L}}
\newcommand{\bfM}{\mathbf{M}}
\newcommand{\bfN}{\mathbf{N}}
\newcommand{\bfO}{\mathbf{O}}
\newcommand{\bfP}{\mathbf{P}}
\newcommand{\bfQ}{\mathbf{Q}}
\newcommand{\bfR}{\mathbf{R}}
\newcommand{\bfS}{\mathbf{S}}
\newcommand{\bfT}{\mathbf{T}}
\newcommand{\bfU}{\mathbf{U}}
\newcommand{\bfV}{\mathbf{V}}
\newcommand{\bfW}{\mathbf{W}}
\newcommand{\bfX}{\mathbf{X}}
\newcommand{\bfY}{\mathbf{Y}}
\newcommand{\bfZ}{\mathbf{Z}}

\newcommand{\sfL}{\mathcal{L}}
\newcommand{\sfD}{\mathcal{D}}
\newcommand{\sfH}{\mathcal{H}}
\newcommand{\sfN}{\mathcal{N}}
\newcommand{\sfA}{\mathcal{A}}
\newcommand{\sfC}{\mathcal{C}}
\newcommand{\sfS}{\mathcal{S}}
\newcommand{\sfO}{\mathcal{O}}
\newcommand{\sfU}{\mathcal{U}}
\newcommand{\sfR}{\mathcal{R}}

\newcommand{\bfa}{\mathbf{a}}
\newcommand{\bfb}{\mathbf{b}}
\newcommand{\bfc}{\mathbf{c}}
\newcommand{\bfd}{\mathbf{d}}
\newcommand{\bfe}{\mathbf{e}}
\newcommand{\bff}{\mathbf{f}}
\newcommand{\bfg}{\mathbf{g}}
\newcommand{\bfh}{\mathbf{h}}
\newcommand{\bfi}{\mathbf{i}}
\newcommand{\bfj}{\mathbf{j}}
\newcommand{\bfl}{\boldsymbol{\ell}}
\newcommand{\bfm}{\mathbf{m}}
\newcommand{\bfn}{\mathbf{n}}
\newcommand{\bfo}{\mathbf{o}}
\newcommand{\bfp}{\mathbf{p}}
\newcommand{\bfq}{\mathbf{q}}
\newcommand{\bfr}{\mathbf{r}}
\newcommand{\bfs}{\mathbf{s}}
\newcommand{\bft}{\mathbf{t}}
\newcommand{\bfu}{\mathbf{u}}
\newcommand{\bfv}{\mathbf{v}}
\newcommand{\bfw}{\mathbf{w}}
\newcommand{\bfx}{\mathbf{x}}
\newcommand{\bfy}{\mathbf{y}}
\newcommand{\bfz}{\mathbf{z}}

\newcommand{\tr}{\operatorname{tr}}
\newcommand{\IL}{\mathbb{L}}
\newcommand{\IM}{\mathbb{M}}
\newcommand{\IQ}{\mathbb{Q}}
\newcommand{\IN}{\mathbb{N}}
\newcommand{\IR}{\mathbb{R}}
\newcommand{\IC}{\mathbb{C}}




==> arXiv v2/problem-setting.tex <==
\section{Problem setting and notations}

We consider Bayesian inverse problems, where we seek a
characterization of the parameter $x\in\mathbb{R}^d$
from observation of data $y$. The parameter $x$ is endowed with
the prior probability density function $\pi_0$.
The law of $x$ conditioned on $y$ is called the posterior
distribution.
Its density is given by the Bayes rule as follow
\begin{equation}
 \pi(x) \propto \mathcal{L}(x) \rho(x),
\end{equation}
where $\mathcal{L}(x)$ is the likelihood function, that is the
probability density function of $y$ conditioned on $x$.
The likelihood
function might be known up to a multiplicative
constant.\todo{paragraph moved to intro}

In a common
configuration the data are defined by $y=f(x)+\xi$ where $f$ is a
forward model and where $\xi\sim\mathcal{N}(0,\Gamma)$ is an additive
Gaussian noise. In this case,
$\mathcal{L}(x)\propto\exp(-\|f(x)-y\|_{\Gamma^{-1}}^2)$.
In the following we will assume $\rho=\mathcal{N}(0,I_d)$.
This is a reasonable assumption as  
many problems with different priors could
be recasted to this setting through an appropriate change of
variables.\todo{db: I propose to remove this paragraph}

We seek approximation to $\pi$ in the form of $T_\sharp\rho$, the
push-forward of $\rho=\mathcal{N}(0,I_d)$
through a diffeomorphism
$T:\mathbb{R}^d\rightarrow\mathbb{R}^d$.
This means $T_\sharp\rho$ is the probability density function of the
random vector $T(Z)$ with $Z\sim\rho$ and it satisfies
$T_\sharp\rho(x) = \rho \circ T^{-1}(x) \vert \nabla T^{-1}(x)
\vert$.
For some prescribed tolerance $\varepsilon>0$,
our goal is to construct a map $T$ such that the Kullback Leibler (KL)
satisfies \todo{paragraph moved to intro}
\begin{equation}
  \Dkl( \pi || T_{\sharp}\rho ) =
  \int\log\left( \frac{\pi(x)}{T_{\sharp}\rho(x)}\right) \pi(x) \d x \leq \varepsilon \;.
\end{equation}

In Section \ref{sec:LazyMaps} we show how to build such a map in a set
of computationally feasible map that we call lazy maps. However, the
complexity to reach \eqref{eq:KLDivergence} might be large if
$\varepsilon$ is too small. In this case, we show in Section
\ref{sec:LayersLazyMaps} how to reach \eqref{eq:KLDivergence} via the
composition of many lazy maps.\todo{moved to intro}

% In Section \ref{sec:LazyMaps} we will restrict our attention to a particular class of maps
% with fixed complexity called lazy maps. This will lead to an algorithm
% aiming to satisfy \eqref{eq:KLDivergence} in one step. The complexity
% of such algorithm 

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> intro_wed530.tex <==
\section{Introduction}

% Inference in the Bayesian setting typically requires the computation of integrals $\int f({x}) \pi({x}) \d{x}$, where $\pi$
% %
% is the density\footnote{In this paper, we only consider distributions that are absolutely
%   continuous with respect to the Lebesgue measure on $\mathbb{R}^d$, and thus
%   will use the notation $\pi$ to denote both the distribution and
%   its associated density.}  
% of some analytically \textit{intractable} (posterior) distribution which is known up to a normalizing constant.
Inference in the Bayesian setting typically requires the computation of integrals $\int f  \, \d\pi$  over an \textit{intractable} posterior distribution whose density\footnote{In this paper, we only consider distributions that are absolutely continuous with respect to the Lebesgue measure on $\mathbb{R}^d$, and thus will use the notation $\pi$ to denote both the distribution and its associated density.} $\pi$ is known up to a normalizing constant.
%
One approach to this problem is to construct a
deterministic nonlinear transformation, i.e., a \emph{transport map}
\cite{villani2008optimal}, \todo{took out the NF mention here since we describe it immediately below}
%, also referred to as a normalizing flow (see \cite{papamakarios2019normalizing,otherNFreview} for an overview), 
that induces a coupling of $\pi$ with a tractable distribution
$\rho$ (e.g., a standard Gaussian).
Formally, we seek a map $T$ that pushes forward $\rho$ to $\pi$, written as $T_\sharp \rho = \pi$, such that the change of variables
$\int f \, \d \pi = \int f \circ T \, \d \rho $ makes integration
tractable.

Many constructions for such maps have been developed in recent years. Normalizing flows (see \cite{rezende2015variational,tabak2013family,papamakarios2019normalizing,kobyzev2020normalizing} and references therein) build transport maps via a deep composition of functions parameterized by neural networks, 
with certain ansatzes 
% while enforcing certain structure
 to enable efficient computation. Many recently proposed autoregressive flows (for example \cite{Kingma2016,jaini2019sum}) compose triangular maps, which allow for efficient evaluation of the Jacobian determinants. In general, triangular maps \cite{bogachev2005triangular,rosenblatt1952remarks,knothe1957contributions} are
sufficiently general to couple any absolutely continuous pair of
distributions $(\rho, \pi)$, and their numerical approximations have
been investigated in \cite{el2012bayesian,marzouk2016introduction, spantini2018inference, Jaini2019}. The flow map of a neural ordinary differential equation \cite{Chen2018,Dupont2019,gholaminejad2019anode} can also been seen as an infinite-layer limit of a normalizing flow.
% that can reduce the complexity of density estimation. 
Alternatively, Stein variational methods \cite{liu2016stein,liu2017stein,Detommaso2018} provide a nonparametric way of constructing $T$ as a composition of functions lying in a chosen RKHS.
%
Many of these constructions are useful not only for variational inference 
%(e.g., approximating $\pi$ by $T_\sharp \rho$ in the sense of Kullback--Leibler (KL) divergence) 
but also for density estimation 
%(i.e., approximating $\pi$ by $\widehat{S}^{-1}_\sharp \rho$ where the map  $\widehat{S} = \widehat{T}^{-1}$  is estimated given a sample from $\pi$)
 \cite{laparra2011iterative,tabak2010density,dinh2016density}. \todo{We could remove this last sentence if tight on space, and scatter the citations around as needed.}

In general, it can be difficult to represent expressive maps in high dimensions. For example, triangular maps on $\mathbb{R}^d$ must describe $d$-variate functions and thus immediately encounter the curse of dimensionality. Similarly, kernel-based methods lose expressiveness in high dimensions \cite{Detommaso2018,Chen2019}. Flow-based methods often increase expressiveness by adding layers, but this is typically performed in an ad hoc or unstructured way, which also requires tuning. \todo{I wanted to convey the idea that layers are added rather generically, in an unfocused way, and that tuning shows up in multiple places.}

Here we propose a framework for inference that creates target-informed architectures around \emph{any} class of transport maps or normalizing flows. In particular, our framework uses rigorous \textit{a priori} error bounds to discover and exploit low-dimensional structure in a given target distribution. It also provides a methodology for efficiently solving high-dimensional inference problems via greedily constructed compositions of \emph{structured} low-dimensional maps. \todo{I think this paragraph is sharper. I wanted to inject the notion of architecture, and highlight the use of a rigorous a priori bound.}

The impact of our approach rests on two observations. 
%
First, the coordinate basis in which one expresses a transport map (i.e., $T(x)$ versus $U T(x)$, where $U$ is a rotation on $\R^d$) can 
% drastically change
strongly affect
% \todo{pretty strong there. OK, or should we say ``significantly affect'' ``strongly affect''}
 the training behavior and final performance of the method. Our framework identifies an ordered basis that best reveals a certain low-dimensional structure in the problem. Expressing the transport map in this basis focuses the expressiveness of the underlying transport class and allows for principled dimension reduction. This basis is identified by minimizing an upper bound on the Kullback--Leibler (KL) divergence between $\pi$ and its approximation, which follows from logarithmic Sobolev inequalities (see \cite{zahm2018certified}) relating the KL divergence to gradients of the target density. % via an {average derivative functional} \cite{samarov1993exploring}.

% mention GREEDY
Second, in the spirit of normalizing flows, we seek to increase the expressiveness of a transport map using repeated compositions. Rather than specifying the length of the flow before training, we increase the length of the flow sequentially. For each layer, we apply the framework above to a \emph{residual} distribution that captures the deviation between the target distribution and its current approximation. We prove weak convergence of this greedy approach to the target distribution under reasonable assumptions. This sequential framework enables efficient layer-wise training of high-dimensional maps, which especially helps control the curse of dimensionality in certain transport classes. As we shall demonstrate empirically, the greedy composition approach can further improve accuracy at the end of training, compared to baseline methods. 


%({\bf I think I capture this section above, except for information on where the bound comes from. I dont think that is needed here.})
% We considers maps are low-dimensional in
%that the transformation is restricted to a low-dimensional subspace of the
%parameter space; thus they are termed ``lazy.'' We identify the low-dimensional subspaces sequentially, by greedily minimizing a bound on the KL divergence between $\pi$ and its approximation. The bound itself follows from
%logarithmic Sobolev inequalites (see \cite{zahm2018certified})
%relating the KL divergence to gradients of the target density. We
%prove weak convergence of this approach to the target distribution,
%given even suboptimal choices of the subspace.
%
%


%{\bf I'm not sure if we need to this, it seems out of context in the intro (they don't know what low dimensional structure is yet) -->}
%We point out that while the lazy framework is able to identify and efficient capture exact low dimensional structure in a problem, the overall approach does not require the problem to be specifically structured. We also emphasize that our overall approach does not require any \emph{global} low dimensionality in the likelihood function (as in \cite{cui2014likelihood,Chen2019}, for example).%: rather, it can converge even for maps that act on a single direction at a time, despite $\pi$ and $\rho$ differing in all directions.

% despite the difference between $\pi$ and $\rho$ not being confined to a low-dimensional subspace. 


% \section{Preliminaries}

\paragraph{Preliminaries.} We will consider target distributions with densities $\pi$ on $\mathbb{R}^d$ that are differentiable almost everywhere and that can be evaluated up to a normalizing constant. Such a target will often be the posterior of a Bayesian inference problem, e.g.,
\begin{equation}\label{eq:PosteriorDensity}
 \pi(x) \coloneqq p(x\vert y) \propto \mathcal{L}_y(x) \pi_0(x),
\end{equation}
where $\mathcal{L}_y(x) \coloneqq p(y \vert x)$ is the likelihood function and $\pi_0$ is the prior. We denote the standard Gaussian density on $\mathbb{R}^d$ as $\rho$. We will consider maps $T: \mathbb{R}^d \to \mathbb{R}^d$ that are diffeomorphisms,\footnote{In general $T$ does not need to be a diffeomorphism, but only a
  particular invertible map; see Appendix \ref{app:triangular-maps}
  for more details. The distributions we will consider in this paper, however, fulfill the necessary
  conditions for $T$ to be differentiable almost everywhere.}
and with some abuse of notation, we will write the pushforward density of $\rho$ under $T$ as $T_\sharp\rho(x) \coloneqq \rho \circ T^{-1}(x) \vert \nabla T^{-1}(x) \vert$. We will frequently also use the notion of a \emph{pullback} distribution or density, written as $T^\sharp\pi \coloneqq (T^{-1})_\sharp\pi$.

%{\bf Before:}
%Our goal is to find a map $T$ that satisfies  $\Dkl( \pi || T_{\sharp}\rho ) \leq \varepsilon$ for some prescribed tolerance $\varepsilon > 0$. In Section \ref{sec:LazyMaps} we show how to build a single map in the ``lazy'' format described above. However, the map complexity needed to satisfy the prescribed tolerance might be large if $\varepsilon$ is too small. We thus show in Section \ref{sec:LayersLazyMaps} how to improve our approximations by greedily composing many lazy maps.

In \S\ref{sec:LazyMaps} we show how to build a single map in the low-dimensional ``lazy'' format described above, and describe the class of posterior distributions that admit such structure. In \S\ref{sec:LayersLazyMaps} we develop a greedy algorithm for building deep compositions of lazy maps, which effectively decomposes any inference problem into a series of lower-dimensional problems. 
% Each layer of such a map is constructed to transform the base distribution along a subspace we learn to be most important to improving the performance of the map. 
\S\ref{sec:NumericalExamples} presents numerical experiments highlighting the benefits of the lazy framework.
%
While our numerical experiments employ inverse autoregressive flows \cite{IAF} and polynomial transport maps \cite{SoS,us} as the underlying transport classes, we emphasize that the lazy framework is applicable to any class of transport. The complexity of the map, and hence the computational effort, can be tailored at each layer, making the method exceptionally flexible. \todo{Possibly omit one or two last sentences.}


%% REVISED STUFF ABOVE
% %% OLD STUFF (source material) BELOW


% \begin{itemize}
% \item Underlying idea: what kind of \emph{structure} in inference
%   problems does this take advantage of? Beyond just low-rank in the
%   LIS sense. No assumption of low-dimensionality in the likelihood;
%   convergence (given condition on $t$) for even $r=1$. Relationship to
%   matching pursuit. \todo{OZ fills in here!}
% \item Generality of the method; how it can be used. We use lazy triangular
%   maps here, but could do many other things instead.
% \end{itemize}

% \todo[inline]{OLD INTRO STARTS HERE}

% The solution of many sstatistical inference problems require the
% evaluation of integrals $I[f]=\int f({x}) \pi(\d{x})$
% with respect to some \textit{intractable} distribution $\pi$\footnote{
%   In the following we will consider only distributions $\pi$ that have a
%   Radon–Nikodym derivative with respect to the Lebesgue measure, and
%   will use the notation $\pi$ to refer to both the distribution and
%   the associated density.
% }.
% The intractability of the distribution $\pi$ is to be intended as 
% the inability to generate a sample
% $\{{x}_i\}_{i=1}^n \iidsim \pi$
% with a computational time that is proportional to the generation of an
% i.i.d. sample from $\mathcal{N}(0,{\bf I}_d)$.
% In turn, this renders the Monte-Carlo approximation
% $I[f]\approx \mathcal{Q}_n[f] := n^{-1} \sum_{i=1}^{n}f({x}_i)$
% challenging.

% These distributions often occur in problems of inference of a
% parameter $x$, where
% the non-trivial assimilation of evidence $y$ can result in a complex
% update of the prior belief $\pi(x)$ through the Bayes rule
% \begin{equation}\label{eq:PosteriorDensity}
%  \pi(x\vert y) \propto \mathcal{L}_y(x) \pi(x),
% \end{equation}
% where $\mathcal{L}(x)$ is the likelihood function, that is the
% probability density function of $y$ conditioned on $x$.
% Likelihood functions are often known up to a multiplicative constant,
% which further complicates the task of generating samples from $\pi$.

% We tackle this problem by the identification of a
% diffeomorphism\footnote{
%   In general $T$ does not need to be a diffeomorphism, but only a
%   particular invertible map; see Appendix \ref{app:triangular-maps}
%   for more details. The distributions we will consider in this paper, however, fulfill the necessary
%   conditions for $T$ to be differentiable almost everywhere.
% }
% $T:\mathbb{R}^d\rightarrow\mathbb{R}^d$ characterizing the coupling
% $(\rho,\pi)$ between a \textit{tractable} distribution $\rho$ 
% and the intractable distribution $\pi$,
% meaning that $T$ is such that $\rho(A)=\pi(T(A))$ for any measurable set $A$.
% We will say that the transport $T$ \textit{pushes-forward}
% the distribution $\rho$ to the distribution $\pi$,
% and we will write $T_\sharp\rho=\pi$.
% By an abuse of notation the density associated to $\pi$ is has the
% form $T_\sharp\rho := \rho \circ T^{-1}(x) \vert \nabla T^{-1}(x)
% \vert$.
% We will equivalently say that $T$ \textit{pulls-back} the
% distribution $\pi$ to the distribution $\rho$ and write
% $T^\sharp\pi(x) := (T^{-1})_\sharp\pi(x)$.

% The availability of the transport $T$ renders the integration with respect to
% $\pi$ tractable, in fact it defines the change of variables
% $I[f]=\int f({x}) \pi(\d{x}) = \int f \circ T({x}) \rho(\d{x})$,
% which results in an integral with respect to the tractable distribution
% $\rho$.
% The distribution $\rho$ is a degree of freedom of the problem, and
% its choice, as we will see in the following,
% is driven by computational and practical requirements.

% In general there exist many maps such that $T_\sharp\rho=\pi$, but for
% practical reasons only maps with specific structures are
% computationally tractable: a non exhaustive list includes triangular
% transport maps
% \cite{el2012bayesian,spantini2018inference,bigoni2016nips},
% normalizing flows \cite{tabak2013family,rezende2015variational},
% Stein flows \cite{liu2016stein,Detommaso2018,Chen2019},
% autoregressive flows \cite{Kingma2016},
% neural ordinary differential equations \cite{Chen2018,Dupont2019}
% \todo{DB: add some literature (normalizing flow)}.
% The choice of a particular class of transports depends from its
% approximation power as well as the cost selected to identify the
% one such that $T_\sharp\rho\approx\pi$.

% In this work we will seek $T$ in a
% class of low-dimensional transport maps whose action is confined to
% carefully selected subspaces of the parameter space.
% For some prescribed tolerance $\varepsilon>0$,
% our goal is to find a map $T$ in this approximation class,
% such that the Kullback-Leibler (KL) divergence satisfies
% \begin{equation}\label{eq:KLDivergence}
%   \Dkl( \pi || T_{\sharp}\rho ) =
%   \int\log\left( \frac{\pi(x)}{T_{\sharp}\rho(x)}\right) \pi(x) \d x \leq \varepsilon \;.
% \end{equation}

% In Section \ref{sec:LazyMaps} we show how to build such a map in a set of computationally feasible map that we call lazy maps. However, the complexity to reach \eqref{eq:KLDivergence} might be large if $\varepsilon$ is too small. In this case, we show in Section \ref{sec:LayersLazyMaps} how to reach \eqref{eq:KLDivergence} via the composition of many lazy maps.


% Because of the greedy/sequential approach, we don't need to put lots of effort into approximating $H$. 




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> layers-lazy-mapsCONF.tex <==
\section{Layers of lazy maps}\label{sec:LayersLazyMaps}


\begin{algorithm}[t]
  \caption{
    Compute layers of lazy maps
  }
  \begin{algorithmic}[1]
    \Procedure{LayersOfLazyMaps}{$\pi$, $\rho$, $\varepsilon$, $r$, $\ell_{{\text{max}}}$}
    \State Set $\pi_0=\pi$ and $\ell=0$
    \While{$\ell \leq \ell_{{\text{max}}}$ and $\frac{1}{2}\trace(H_{\ell})\geq \varepsilon$}
        \State $\ell\gets\ell+1$
        \State Compute $T_\ell  = $ \textsc{LazyMap}($\pi_{\ell-1}$, $\rho$, $0$, $r$) \Comment{Algorithm \ref{alg:LazyMap}} 
        \State Update $\frak{T}_{\ell}=\frak{T}_{\ell-1}\circ T_\ell$ 
        \State Compute $\pi_\ell = (\frak{T}_{\ell})^\sharp \pi$ 
        \State Compute $H_{\ell}=\int (\nabla\log\frac{\pi_\ell}{\rho} )(\nabla\log\frac{\pi_\ell}{\rho} )^\top\d\pi_\ell$
    \EndWhile
    
    \State\Return $\frak{T}_\ell=T_1\circ\cdots\circ T_\ell$
    \EndProcedure
  \end{algorithmic}\label{alg:LayersOfLazyMaps}
\end{algorithm}



The restriction $r\leq r_{{\text{max}}}$ in Algorithm \ref{alg:LazyMap} helps control the computational cost of constructing the lazy map, but unless a problem admits sufficient lazy structure, $T_\sharp\rho$ may not adequately approximate the posterior. To extend the numerical benefits of the lazy framework to general problems, we consider the ``deeply lazy'' map $\frak{T}_\ell$, a composition of $\ell$ lazy maps:
\[
 \frak{T}_\ell = T_1\circ\hdots\circ T_\ell ,
 \quad T_k \in\mathcal{T}_{r}(U^{k}) ,
\]
where each $T_k$ is a lazy map associated with a different unitary matrix $U^k\in\R^{d\times d}$.
For simplicity we consider the case where each lazy layer $T_k$ has the same rank $r$,
%$r = r_{{\text{max}}}$, 
though it is trivial to allow the ranks to vary from layer to layer.

In general, the composition of lazy maps is not itself a lazy map. For example, there exists $U^1\neq U^2$ such that $\frak{T}_2=T_1\circ T_2$ might depend nonlinearly on each input variable and so it cannot be written as in \eqref{eq:LazyMap}. Also, approximations of the form of $(\frak{T}_\ell)_\sharp\rho$ are different than those constructed by projection pursuit \cite{huber1985projection}.\todo{Maybe we have have an explanation in an appendix} %
% We note that are different than those constructed by projection pursuit \cite{huber1985projection}
%Notice also that there is no chance in general to write $(\frak{T}_\ell)_\sharp\rho(x)$ as a product $f_1( U^{1\top}_{r} x) \cdots f_\ell( U^{\ell \top}_{r} x)\rho(x)$; otherwise, by Proposition \ref{prop:CaracterizationOfLazyMaps}, $\frak{T}_\ell$ would be a lazy map with rank bounded by $r \ell$. As a consequence, approximations of the form of $(\frak{T}_\ell)_\sharp\rho$ are different than those constructed by projection pursuit \cite{huber1985projection}.

The diagnostic matrix $H$ allows us to build deeply lazy maps in a greedy way.
After $\ell-1$ iterations, the composition of maps
$\frak{T}_{\ell-1}=T_1\circ\hdots\circ T_{\ell-1}$ has been
constructed.
We seek a unitary matrix $U^{\ell}\in\R^{d\times d}$ and a lazy map $T_{\ell}\in\mathcal{T}_r(U^{\ell})$ such that $(\frak{T}_{\ell-1} \circ  T_\ell)_\sharp\rho$ best improves over  $(\frak{T}_{\ell-1})_\sharp\rho$ as an approximation to the posterior. To this end, we define the residual distribution
\[ 
\pi_{\ell-1} = (\frak{T}_{\ell-1})^\sharp \pi,
\]
i.e., the pullback of $\pi$ through the current transport map $\frak{T}_{\ell-1}$.
Note that $\Dkl( \pi||(\frak{T}_{\ell-1} \circ  T_\ell)_\sharp \rho) = \Dkl( \pi_{\ell-1} ||(T_\ell)_\sharp \rho)$. We thus build $T_\ell$ using Algorithm \ref{alg:LazyMap}, replacing the posterior $\pi$ by the residual distribution $\pi_{\ell-1}$.
We then update the transport map to be $\frak{T}_{\ell}=\frak{T}_{\ell-1}\circ T_\ell$ and the residual density $\pi_\ell = (\frak{T}_{\ell})^\sharp \pi$. 


We note that applying Proposition \ref{prop:LogSobResult} to $\pi_\ell$ with $r=0$ yields
 \[
 \Dkl(\pi||(\frak{T}_\ell)_\sharp\rho)=\Dkl(\pi_\ell||\rho)\leq \frac{1}{2}(\lambda_1+\cdots+\lambda_d)=\frac{1}{2}\trace(H_{\ell}),
 \]
 where we define the diagnostic matrix at iteration $\ell$ as, 
\[ 
H_{\ell}=\int \left (\nabla\log\frac{\pi_\ell}{\rho} \right ) \left (\nabla\log\frac{\pi_\ell}{\rho}  \right )^\top\d\pi_\ell.
\]
%
We see that $\frac12 \trace{(H_\ell)}$ provides an independently useful error bound \todo{Sharpen further? Want to highlight that this is a new and very broadly applicable bound, of independent interest!} on the forward KL divergence, applicable to \emph{any} flow-based method. Here it can be used as a stopping criterion for the greedy algorithm: continue adding layers until the bound falls below some desired threshold. 
%
This construction is summarized in Algorithm \ref{alg:LayersOfLazyMaps}, and details on its numerical implementation are given in Appendix~\ref{app:numerical-algorithms}.

%  (As written, this algorithm would compute the matrix $H_\ell$ twice: once in step 8
% and once in step 2 of Algorithm \ref{alg:LazyMap} at the next
% iteration. Of course, the actual implementation of this algorithm
% reuses this information.)\todo{db: we may find a
%   way to remove the last two sentences and maybe refer to the actual
%   implementation in the appendix?}



The next proposition gives a sufficient condition on $U^\ell$ to guarantee the convergence of our greedy algorithm. The proof is given in Appendix \ref{proof:GreedyConvergence_condition}.
\begin{proposition}\label{prop:GreedyConvergence_condition}
 Let $U^1,U^2,\hdots$ be a sequence of unitary matrices.
 For any $\ell\geq1$, we let $T_\ell \in\mathcal{T}_r(U^\ell)$ be a lazy map that minimizes $\Dkl( \pi_{\ell-1} ||(T_\ell)_\sharp \rho)$, where $\pi_{\ell-1} = (T_1\circ\hdots\circ T_{\ell-1})^\sharp \pi$.
 If there exists $0< t\leq 1$ such that for any $\ell\geq1$
 \begin{equation}\label{eq:GreedyConvergence_condition}
  \Dkl( (U_r^{\ell \top})_\sharp \pi_{\ell-1} || \rho_r )
  \,\geq\, t  \sup_{\substack{ U\in\R^{d\times d} \\ \text{s.t.} UU^\top=I_d}} \Dkl( (U_r^\top)_\sharp \pi_{\ell-1} || \rho_r ),
 \end{equation}
 
 then $(T_1\circ\hdots\circ T_\ell)_\sharp\rho $ converges weakly to $\pi$.
\end{proposition}

Let us comment on the condition \eqref{eq:GreedyConvergence_condition}. Recall that the unitary matrix $U$ that maximizes $\Dkl( (U_r^\top)_\sharp \pi_{\ell-1} || \rho_r )$ is optimal; see \eqref{eq:KL_Tstar_Decomp}.
 % with $\pi$ replaced by $\pi_{\ell-1}$
By \eqref{eq:GreedyConvergence_condition}, the case $t=1$ means that $U^\ell$ is optimal at each iteration. This corresponds to an
\textit{ideal} greedy algorithm. The case $0<t<1$ allows suboptimal
choices for $U^\ell$ without losing the convergence property of the
algorithm. Such a \textit{weak} greedy algorithm converges even with a
potentially crude selection of $U^\ell$ that corresponds to a $t$
close to zero. This also is why an approximation to
$H_\ell$ is expected to be sufficient; see Section
\ref{sec:NumericalExamples}.
% \todo{we write this concept twice, also in the previous section. YM: that's okay!}
Following \cite{Temlyakov2011}, one can further relax the
condition \eqref{eq:GreedyConvergence_condition} by replacing $t$ with a
non-constant parameter $t_\ell$ which can go to zero under certain conditions. This development is left for future work.
Finally let us note that Proposition \ref{prop:GreedyConvergence_condition} does not require any constraints on $r$, so we have convergence even with $r=1$, where each layer only acts on a single direction at a time. %Of course, larger $r$ yields faster convergence





%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> problem-setting.tex <==
\section{Problem setting and notations}

We consider Bayesian inverse problems, where we seek a
characterization of the parameter $x\in\mathbb{R}^d$
from observation of data $y$. The parameter $x$ is endowed with
the prior probability density function $\pi_0$.
The law of $x$ conditioned on $y$ is called the posterior
distribution.
Its density is given by the Bayes rule as follow
\begin{equation}
 \pi(x) \propto \mathcal{L}(x) \rho(x),
\end{equation}
where $\mathcal{L}(x)$ is the likelihood function, that is the
probability density function of $y$ conditioned on $x$.
The likelihood
function might be known up to a multiplicative
constant.\todo{paragraph moved to intro}

In a common
configuration the data are defined by $y=f(x)+\xi$ where $f$ is a
forward model and where $\xi\sim\mathcal{N}(0,\Gamma)$ is an additive
Gaussian noise. In this case,
$\mathcal{L}(x)\propto\exp(-\|f(x)-y\|_{\Gamma^{-1}}^2)$.
In the following we will assume $\rho=\mathcal{N}(0,I_d)$.
This is a reasonable assumption as  
many problems with different priors could
be recasted to this setting through an appropriate change of
variables.\todo{db: I propose to remove this paragraph}

We seek approximation to $\pi$ in the form of $T_\sharp\rho$, the
push-forward of $\rho=\mathcal{N}(0,I_d)$
through a diffeomorphism
$T:\mathbb{R}^d\rightarrow\mathbb{R}^d$.
This means $T_\sharp\rho$ is the probability density function of the
random vector $T(Z)$ with $Z\sim\rho$ and it satisfies
$T_\sharp\rho(x) = \rho \circ T^{-1}(x) \vert \nabla T^{-1}(x)
\vert$.
For some prescribed tolerance $\varepsilon>0$,
our goal is to construct a map $T$ such that the Kullback Leibler (KL)
satisfies \todo{paragraph moved to intro}
\begin{equation}
  \Dkl( \pi || T_{\sharp}\rho ) =
  \int\log\left( \frac{\pi(x)}{T_{\sharp}\rho(x)}\right) \pi(x) \d x \leq \varepsilon \;.
\end{equation}

In Section \ref{sec:LazyMaps} we show how to build such a map in a set
of computationally feasible map that we call lazy maps. However, the
complexity to reach \eqref{eq:KLDivergence} might be large if
$\varepsilon$ is too small. In this case, we show in Section
\ref{sec:LayersLazyMaps} how to reach \eqref{eq:KLDivergence} via the
composition of many lazy maps.\todo{moved to intro}

% In Section \ref{sec:LazyMaps} we will restrict our attention to a particular class of maps
% with fixed complexity called lazy maps. This will lead to an algorithm
% aiming to satisfy \eqref{eq:KLDivergence} in one step. The complexity
% of such algorithm 

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

